Memory Efficient Optimizers with 4-bit States

Optimizer states are a major source of memory consumption for training neural networks, limiting the maximum trainable model within given memory budget. Compressing the optimizer states from 32-bit floating points to lower bitwidth is promising to reduce the training memory footprint, while the current lowest achievable bitwidth is 8-bit. In this work, we push optimizer states bitwidth down to 4-bit through a detailed empirical analysis of first and second moments. Specifically, we find that moments have complicated outlier patterns, that current block-wise quantization cannot accurately approximate. We use a smaller block size and propose to utilize both row-wise and column-wise information for better quantization. We further identify a zero point problem of quantizing the second moment, and solve this problem with a linear quantizer that excludes the zero point. Our 4-bit optimizers are evaluated on a wide variety of benchmarks including natural language understanding, machine translation, image classification, and instruction tuning. On all the tasks our optimizers can achieve comparable accuracy with their full-precision counterparts, while enjoying better memory efficiency.

==> definition.tex <==
\section{Background}

\newcommand{\oneb}{\mathbf{1}}

\subsection{Integer Matrix Multiplication}
Let $\Nb_b=\{0, \dots, 2^b-1\}$ be the set of all $b$-bit integers. Given two matrices $\bar\Xv\in \Rb^{N\times K}$ and $\bar\Wv\in \Rb^{K\times L}$, where we approximate as
\begin{align*}
\bar\Xv \approx s_X \Xv + b_X\oneb,~~~~ \bar\Wv \approx s_W \Wv + b_W,
\end{align*}
where $s_X, b_X, s_W, b_W$ are real-valued scalars, and all the elements of $\Xv, \Wv$ belong to $\Nb_b$. 

We can approximate 
\begin{align*}
&\bar\Yv = \bar\Xv \bar\Wv\approx (s_X \Xv + b_X\oneb)(s_W \Wv + b_W) \\
=&s_Xs_W \Xv\Wv + b_Xs_W \oneb_N (\oneb_K^\top \Wv) + s_Xb_W(X\oneb_K)\oneb_L^\top + b_Nb_WK \oneb_N\oneb_L^\top \\
=& \hat\Yv \approx s_Y \Yv + b_Y.
\end{align*}
To compute $s_Y, \Yv$ and $b_Y$, there involves two steps
\begin{enumerate}
    \item compute \emph{integer} matrix product $\Xv\Wv$, $\oneb_N (\oneb_K^\top \Wv)$, and $(X\oneb_K)\oneb_L^\top$; 
    \item compute $\hat\Yv$ in \emph{floating points}, compute $s_Y$ and $b_Y$, and quantize $$\Yv=\mathrm{round}(\mathrm{clip}((\hat\Yv-b_Y)/s_Y, 0, 2^b-1)).$$
\end{enumerate}

\section{Theory}
\subsection{Binary Neural Networks}
Binary neural networks (BNNs) use binary matrix multiplications to compute the activations. However, as their weights and activations are binary, the capacity of BNNs is limited. There lacks a theory on the representation power of BNNs. Questions include:
\begin{enumerate}
    \item Are BNNs universal function approximators?
    \item How large is the approximation error of BNNs, and how does it compare to the error of regular neural networks?
\end{enumerate}

We are trying to address these questions in this work.

\subsection{Generalized Integer Multiplication}
In this part, we give a ``lower bound'' of BNN's representation capacity. We show that for each quantized neural network, there exists a wider BNN that represents exactly the same function. Therefore, BNNs are at least as powerful as quantized neural networks. We show this by construction.

Critically, we consider integer multiplication as the multiplication of two binary strings. Consider the multiplication $y=xw$, where $x, w\in \Nb_b$ and $y\in \Nb_{2b}$.
We can view $x, w$ as $b$-bit binary strings $\xv^b$ and $\yv^b$, where
$$x=\sum_{i=0}^{b-1} 2^i x^b_i,~~~~w=\sum_{i=0}^b 2^i w^b_i.$$
Then, the product
\begin{align}\label{eqn:y}
y=xw=\sum_{i=0}^{b-1}\sum_{j=0}^{b-1} 2^{i+j} (x^b_i\land w^b_i)=\sum_{k=0}^{2b-2} 2^{k} y^b_k, \mbox{ where } y_b^k = \sum_{j=\max\{0, b-1-k\}}^{\min\{k, b-1\}} x^b_j w^b_{k-j}.
\end{align}
We can express the binary string operation as convolution:
$$\yv^b = \xv^b * \wv^b.$$
Alternatively, we can view this as a special case of binary matrix multiplication
$$\yv^b = \Wv^m \xv, \mbox{ where } w^m_{kj} = \Ib(0\le k-j < b) w_{k-j}^b.$$
Note that, the binary matrix $\Wv^m\in \{0, 1\}^{(2b-1)\times b}$ has $b(2b-1)$ degrees of freedom, while the binary string $\wv_b$ only has $b$ degrees of freedom. So the matrix form is much more expressive than the vector form. 

For example, for the computation $y=xw$, where $w=5$, we have
\begin{align*}
\wv^b = (1, 0, 1),~~~~\Wv^m = \begin{bmatrix}
 &  & 1 \\
 & 1 & 0 \\
1 & 0 & 1 \\
0 & 1 &   \\
1 &  &  \\
\end{bmatrix}.
\end{align*}

With general binary matrices, we can generalize integer multiplications. For example,
\begin{align*}
\Wv^m = \begin{bmatrix}
1 & 0 & 1 \\
0 & 1 & 1 \\
0 & 0 & 1 \\ 
1 & 0 & 0 \\
0 & 1 & 0
\end{bmatrix}
\end{align*}
defines a multiplication table as\\ 
\begin{tabular}{cc|cc}
\hline
$x$  & $\xv^b$  & $\yv^b = \Wv^m \xv^b$ & $y$ \\
\hline
0 & (0 0 0) & (0 0 0 0 0) & 0 \\
1 & (1 0 0) & (1 0 0 1 0) & 9 \\
2 & (0 1 0) & (0 1 0 0 1) & 18 \\
3 & (1 1 0) & (1 1 0 1 1) & 27 \\
4 & (0 0 1) & (1 1 1 0 0) & 7 \\
5 & (1 0 1) & (2 1 1 1 0) & 16 \\
6 & (0 1 1) & (1 2 1 0 1) & 25 \\
7 & (1 1 1) & (2 2 1 1 1) & 34 \\
\hline
\end{tabular}

After having the output vector $\yv^b$, we need to convert it to integer $y$, and quantize $y$ back to a $b$-bit binary string $\yv^o$, where
\begin{align*}
y = \sum_{k=0}^{2b-2} 2^{k} y^b_k,~~~~\hat y = \mathrm{round}(\mathrm{clip((y - b_y)/s_y, 0, 2^b-1)}),~~~~
y^o_i = \lfloor \hat y / 2^i \rfloor \mathrm{mod} 2.
\end{align*}

More generally, we can express it in vector format
\begin{align*}
y = \vv^\top \yv^b, ~~~ \yv^o = \lfloor \mathrm{clip((y - \bv)/\sv, 0, \rv)} \rfloor \mathrm{mod} 2.
\end{align*}
or matrix format
\begin{align*}
\yv^o = \mathrm{round}(\mathrm{clip(\Sv (\yv^b - \bv), 0, \rv)}) \mathrm{mod} 2
\end{align*}

\subsection{Binary Neural Networks}

\subsection{Case Study: Representing Comb Functions}

\section{Binary Dot Product}
Consider the dot product $<\av, \bv>$, where $\av, \bv\in \Rb^{N}$.
Let $\alpha=\max_i |a_i|$ and $\tilde a_i=a_i/\alpha$. Define the randomly binarized variable
$$\hat \alpha_i=\begin{cases}
1 & \mbox{w.p. }\frac{\tilde \alpha_i+1}{2}\\
-1 & \mbox{otherwise}.
\end{cases}$$
We have 
$$\E{\hat\alpha_i}=\frac{\tilde \alpha_i+1}{2}-1+\frac{\tilde \alpha_i+1}{2}=\tilde\alpha.$$
Apparently, 
$$\E{<\alpha\hat\av,\beta\hat\bv>}=\alpha\beta\sum_i\E{\hat a_i}\E{\hat b_i}=<\av, \bv>.$$
Furthermore, 
\begin{align*}
\Var{<\hat\av, \hat\bv>}=\sum_i\Var{\hat a_i\hat b_i}
=\sum_i \E{(\hat a_i\hat b_i)^2} - (\tilde a_i \tilde b_i)^2
=\sum_i (1 - \tilde a_i^2 \tilde b_i^2).
\end{align*}
Therefore,
$$\E{(<\av, \bv>-<\alpha\hat\av, \beta\hat\bv>)^2}=\Var{<\alpha\hat\av, \beta\hat\bv>}=\sum_i (\alpha^2\beta^2 - a_i^2b_i^2)$$

\subsection{Deterministic Biased Binarization (XNOR-Net)}
Alternatively, we can choose $\alpha, \beta, \hat\av, \hat\bv$ to 
$$\min_{\alpha,\hat\av}\norm{\av - \alpha\hat\av}_2^2.$$
The solution is 
$$\hat\av=\sign(\av), \alpha=\norm{\av}_1/N, \hat\bv=\sign(\bv), \beta=\norm{\bv}_1/N.$$

Then, 
\begin{align*}
(<\av, \bv>-<\alpha\hat\av, \beta\hat\bv>)^2
= 
\end{align*}

\section{Binary Matrix Multiplication}
\subsection{Unbiased Stochastic}
Consider the matrix product $\Cv=\Av\Bv$. Let $\alpha=\max_{ij} |a_{ij}|, \beta=\max_{ij} |b_{ij}|$ and $\tilde\Av=\Av/\alpha, \tilde\Bv=\Bv/\beta$.
Let $\hat\Av$ and $\hat\Bv$ be the unbiased binarization of $\tilde\Av$ and $\tilde\Bv$.

\begin{align*}
\Var{\alpha\beta\hat\Av\hat\Bv}
= \alpha^2\beta^2\sum_{ij} \Var{\hat\Av_{i,:}\hat\Bv_{:,j}}
= \sum_{ijk}(\alpha^2\beta^2 -  a_{ik}^2 b_{kj}^2)
\end{align*}

\subsection{Biased Deterministic}




\section{Theoretical Formulation}
Let $\Nc_{H, W, B}$ be the function family formed by all $H$-layer, $W$-neuron ReLU networks with $B$-bit activation and weight. 

\subsection{Function Approximation}
\begin{theorem}
For any function $f: [0, 1]^D\rightarrow \{0, 1\}$, which is $L$-Lipschitz continuous. For a fixed neural network family $\Nc_{H, W, B}$, there exist a network $h\in \Nc_{H, W, B}$, such that
\begin{align*}
\norm{f - h} \le \epsilon(H, W, B, D, L).
\end{align*}
\end{theorem}
We would like to find out how does the approximation error relates with $H, W, B, D, L$. Particularly, under certain resource budget, do we favor large $W$ and small $B$, or small $W$ and large $B$.

\noindent\textbf{Caveat: } Existing function approximation theorems are nothing more than enumerating the cells in a high-dimensional grid. This is clearly not how neural networks work in practice.

\subsection{Knowledge Distillation}
The Lipschitz continuous function family might be too large and uninformative. Instead, we can take a knowledge distillation approach:
\begin{theorem}
For any function $f: [0, 1]^D\rightarrow \{0, 1\}\in
\Nc_{H, W_0, \infty}$, and a fixed neural network family $\Nc_{H, W, B}$, there exist a network $h\in \Nc_{H, W, B}$, such that 
\begin{align*}
\norm{f - h} \le \epsilon(H, W, B, D, W_0).
\end{align*}
\end{theorem}
This formulation considers how to approximate an accurate yet huge network in an efficient manner. Existing structural pruning and post-training quantization theory closely relate to this formulation.

\section{2-Layer Neural Networks}
\begin{align*}
\zv = \sigma(\Wv \xv),~~~y=\av^\top\zv.
\end{align*}
Approximate
\begin{align*}
y = \frac{N}{M}\sum_{i\in \Sc} a_i Q(z_i).
\end{align*}
Then,
\begin{align*}
\Var{y} = \E{\Varcond{y}{Q}} + \Var{\Econd{y}{Q}}
= \E{\Varcond{y}{Q}} + \Var{\sum_{i} a_i Q(z_i)},
\end{align*}
where 
\begin{align*}
\Varcond{y}{Q} &= \Econd{y^2}{Q} - \Econd{y}{Q}^2
= \frac{N^2}{M^2}\left(
M(M-1) \frac{y^2}{N^2} + M\E{a_i^2 Q(z_i)^2}
\right) - \Econd{y}{Q}^2\\
=& \frac{M-1}{M} y^2 + \frac{N}{M}\sum_i a_i^2 Q(z_i)^2 - y^2 = \frac{N}{M}\sum_i a_i^2 Q(z_i)^2 - \frac{1}{M}y^2,
\end{align*}
and
\begin{align*}
\Var{\sum_i a_i Q(z_i)} = \sum_i a_i^2 \Var{Q(z_i)}.
\end{align*}
so
\begin{align*}
\Var{y} =& \frac{N}{M}\sum_i a_i^2 \E{Q(z_i)^2} - \frac{1}{M}y^2
+ \sum_i a_i^2 \Var{Q(z_i)} \\
=& \frac{N}{M}\sum_i a_i^2 (z_i^2 + \Var{Q(z_i)}) - \frac{1}{M}y^2
+ \sum_i a_i^2 \Var{Q(z_i)} \\
=& \underbrace{(\frac{N}{M}+1)\sum_i a_i^2 \Var{Q(z_i)}}_{\mbox{\scriptsize Quantization Variance}} + \underbrace{\frac{1}{M}(N\sum_i a_i^2 z_i^2 - y^2)}_{\mbox{\scriptsize Sampling Variance}}
\end{align*}
Assume that $y^2 \ll N\sum_i a_i^2 z_i^2$, and $M \ll N$, then
\begin{align*}
\Var{y}\approx \frac{N}{M}\sum_i a_i^2 (z_i^2 + \Var{Q(z_i)}).
\end{align*}
Therefore, we should pick smallest $B$ and largest $M$ so that $z_i^2$ and $\Var{Q(z_i)}$ are roughly on the same magnitude. 

To minimize the variance, given a total bit budget $b$, we approximately solve
\begin{align*}
\min_B b \sum_i a_i^2 (z_i^2 + V_i/2^b).
\end{align*}


==> garbage.tex <==

\section{Layers}
\subsection{Linear layers}
For linear layers $\Hl{l} = \Hl{l-1}\Thetal{l}$, the gradient is 
\begin{align*}
\nabla_{\Hl{l-1}} = \nabla_{\Hl{l}}\Thetal{l}^\top,\quad
\nabla_{\Thetal{l}} = \Hl{l-1}^\top \nabla_{\Hl{l}},
\end{align*}
One-bit neural network is equivalent with a quantization algorithm, which quantizes $\nabla_{\hl{i}}$ with $b_i$ bits. 
Suppose for $\nabla_{\hl{i}}$, the quantized representation is $\nabla_{\hl{i}}\approx \av_i \beta_i + \mu_i$, where each $\av_i$ is an unsigned $b_i$-bit integer, we further decompose it as
\begin{align*}
\nabla_{\hl{i}}\approx \av_i \beta_i + \mu_i = \beta_i \sum_{j=0}^{b_i-1} \av_{ij} 2^{j} + \mu_i. 
\end{align*}
We construct the quantized representation $\Av$ and a scale matrix and a shift matrix as follows
\begin{align*}
\Av = \begin{bmatrix}
\av_{11}\\
\dots\\
\av_{1b_1}\\
\av_{21}\\
\dots\\
\av_{2b_2}\\
\av_{N1}\\
\dots\\
\av_{Nb_N}\\
\end{bmatrix}
,\quad \gammav = \begin{bmatrix}
\gamma_1 2^0 & \dots & \gamma_1 2^{b_1-1} & & & \\
& & & \gamma_2 2^0 & \dots & \gamma_2 2^{b_2-1} & \\
& & &  &  &  & \dots\\
\end{bmatrix},\quad 
\betav = \begin{bmatrix}
\beta_1\\
\dots\\
\beta_N
\end{bmatrix},
\end{align*}
where $\Av$ is $\sum_i b_i\dots D$-dimensional, $\gammav$ is $N\times \sum_i b_i$-dimensional, and $\betav$ is $N$-dimensional. We can verify that 
\begin{align*}
(\gammav \Av + \betav) \Thetal{l}^\top 
\approx \nabla_{\Hl{l}}\Thetal{l}^\top.
\end{align*}
If the weight $\Thetal{l}$ is binary, then $\Av\Thetal{l}^\top$ only involves \texttt{and} operations and \texttt{popcount} operations. 

To select $b_i$, we derive the variance as 
\begin{align*}
\Var{\nabla_{\Hl{l-1}}}
= \sum_i \Var{(\av_i \beta_i + \mu_i)\Thetal{l}^\top}
= \sum_i \beta_i^2 \Var{\av_i\Thetal{l}^\top}
\le \norm{\Thetal{l}}_F^2 \sum_i \frac{R(\nabla_{\hl{l}})^2}{4B_i^2},
\end{align*}
where $B_i=2^{b_i}-1$, and we can minimize the variance under a given bit budget.

\section{One-bit Linear Algebra}

Considering the multiplication of two matrices $\Av\in \Rb^{N\times K}$ and $\Bv\in \Rb^{K\times M}$. We quantize each row of $\Av$, and each column of $\Bv$ separately, where $b^A_i$ is the numerical precision of $\Av$, and $b^{B}_j$ is the numerical precision of $\Bv$. 

Suppose $\av_i$ and $\bv_{:,j}$ is quantized as 
\begin{align*}
\av_i = \gamma_i^A \sum_{e=0}^{b_i^A - 1} \av_{ie} 2^e, \quad 
\bv_{:j} = \gamma_j^B \sum_{e=0}^{b_j^B - 1} \bv_{je} 2^e.
\end{align*}
Then
\begin{align*}
\av_i \bv_{:j} = \gamma_i^A\gamma_j^B\sum_{e^A=0}^{b_i^A - 1}\sum_{e^B=0}^{b_j^B - 1} \av_{ie^A} 2^{e^A}
 \bv_{je^B} 2^{e^B}.
\end{align*}

\textbf{Uniform quantization} 
If both matrices are uniformly quantized to $b$-bits. Quantized matrix multiplication involves $KNM$ MAC operations in INT$b$. In AVX512 CPUs, this should be $KNMb/256$ instructions. (Intel has dedicated INT8 vector MAC instruction, in the instruction set VNNI).

\textbf{1-bit quantization}
It takes $K (\sum_i b^A_i)(\sum_j b^B_j)$ 1-bit and-popcount (AP) operations. In AVX512 CPUs, this would be be $K (\sum_i b^A_i)(\sum_j b^B_j)/256$ operations in total. 

An Xeon 8380H CPU has 28 cores with 2.9GHz base frequency. Assuming the IPC is 1. It would give us $28\times 2.9GHz = 81.2$G AVX512 ops per second. If $\sum_i b^A_i=4N$ and $\sum_j b^B_j=2M$, it would be equivalent to 5.2Tops. (An ASIC should work much better, since AP operations are much simplier than MAC operations). 


\textbf{Comparison}
If $b_i^A = b^B_j = b$, then 1-bit quantization is $b$ times more expensive than uniform quantization on AVX512 systems. However, I believe by utilizing sparsity we can make $\sum_i b^A_i \approx Nb/2$, so 1-bit quantization is $b/4$ times more expensive. 

\section{Optimization: Reinforce Algorithm}
\begin{align*}
\Hl{l} = Q(\F{l}{\Hl{l-1}, \Thetal{l}}), \Lc=l(\Hl{L}, \Yv)
\end{align*}
\begin{align*}
&\nabla_{\Thetal{l}} \E{l(\Hl{L}, \Yv)}
=\nabla_{\Thetal{l}}\int \prod_{l=1}^L Q(\Hl{l} | \Hl{l-1}, \Thetal{l})
l(\Hl{L}, \Yv) d\Hl{1}\cdots d\Hl{L}\\
=&\int \prod_{l=1}^L Q(\Hl{l} | \Hl{l-1}, \Thetal{l})
\nabla_{\Thetav{l}}\sum_{l=1}^L \log Q(\Hl{l} | \Hl{l-1}, \Thetal{l})
l(\Hl{L}, \Yv) d\Hl{1}\cdots d\Hl{L}\\
=& \E{\nabla_{\Thetav{l}}\sum_{l=1}^L \log Q(\Hl{l} | \Hl{l-1}, \Thetal{l})
l(\Hl{L}, \Yv)}.
\end{align*}
\begin{itemize}
    \item Intuitively, we sample some configurations, if one configuration has large probability and low loss, we move that way.
    \item Zeroth order method, highly ineffective.
    \item We may guide the sampling by straight-through estimator? i.e., first generate a new configuration with the straight-through, then search its neighborhood. 
    \item Use the straight-though as a control variate?
\end{itemize}

\section{Model Capacity}
Suppose we multiply two matrices $\Av\in [2^B-1]^{N\times K}$ and $\Bv\in [2^{B}-1]^{K\times M}$, the result $\Cv\in [2^{2B}-1]^{N\times M}$. Each element $A_{nk}$ is a bit string of length $b$. Denote $A_{nkl}$ be the $l$-th bit.

We have
\begin{align*}
C_{nm} = \sum_{k=0}^{K-1} A_{nk} * B_{km} \Longleftrightarrow
C_{nml} = \sum_{k=0}^{K-1} \sum_{r=0}^{B-1} \Ib(0\le l-r < B) A_{nk,r}B_{km,l-r}
\end{align*}

Alternatively, we can define binary matrices $\bar\Av\in [1]^{N\times KB}$, $\bar\Bv\in [1]^{KB\times 2MB}$, and $\bar\Cv\in [1]^{N\times 2MB}$, let
\begin{align*}
\bar A_{n,k*B+b}=A_{nkb},~~\bar B_{k*B+r,m*B+l}=\Ib(0\le l-r < B) B_{km,l-r}.
\end{align*}
Then, 
\begin{align*}
\bar C=\bar A \bar B \Longleftrightarrow
\bar C_{n,m*B+l} = \sum_{k=0}^{K}\sum_{r=0}^{B-1} \bar A_{n,k*B+r} \bar B_{k*B+r,m*B+l} = 
\sum_{k=0}^{K}\sum_{r=0}^{B-1} A_{nkr} B_{km,l-r} \Ib(0\le l-r < B) = C_{nml}.
\end{align*}

However, Formulation 2 is more flexible where each neuron can have different numerical precision. 

\section{Architecture Design}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> src/3-formulation.tex <==

%In this section, we take SGDM as an example to propose our basic low-precision optimization framework quantizing all model memory during training process.

In this section, we formulate the problem of training neural networks with low precision memory. 
We show that \emph{arithmetic underflow} is the major bottleneck for reducing the numerical precision.
To solve this problem, we propose stochastic quantization and micro-batching techniques.
Here, we mainly consider stochastic gradient descent with momentum (SGDM)~\citep{qian1999momentum, sutskever2013importance} as a motivating example, but the proposed techniques also apply to other optimizers, such as stochastic gradient descent~\citep{bottou2010large} and Adam~\citep{kingma2015adam}.
% \jianfei{distinguish gradient, momentum and model quantizers}

\begin{figure}[t]
    \centering
    \includegraphics[width=.8\linewidth]{figures/diagram.pdf}
    \caption{Dataflow of the LPMM algorithm. Square nodes are in low-precision and kept persistent in memory. Circular nodes are temporary full-precision data, which only consume a small constant-size (dimension-free) buffer. }
    \label{fig:diagram}
\end{figure}


\subsection{Basic Optimization Framework}
Consider the empirical risk minimization problem
\begin{align}
    \label{eq:erm}
    \min_{\theta} f(\theta) = \frac{1}{n} \sum_{i=1}^{n} f_i(\theta),
\end{align}
where $\theta$ is the model parameter. Since the dataset size $n$ is large, stochastic optimizers are adopted for solving the problem. SGDM is one of the most widely used optimizers. Starting with an initial model $\theta_0$ and momentum $m_0=0$, SGDM performs the following updates:
% Currently, the stochastic gradient-based optimization method is standard for training neural network. 
% Some optimizers compute and store the statistics of gradients as their states and provide better performance in practice.
% SGDM(SGD with Momentum) is one of the most commonly used optimizer with state. In usual case, the update rule of SGDM is of the form
\begin{align*}
    m_{t}  \leftarrow \beta m_{t-1} + \nabla \Tilde{f}(\theta_{t-1}),~~~~
    \theta_{t}  \leftarrow \theta_{t-1} - \alpha m_t,
\end{align*}
where $\nabla \Tilde{f}(\theta_{t-1})$ is an unbiased estimator of the gradient. We define
$\nabla \Tilde{f}(\theta_{t-1}):=\nabla f(\theta_{t-1}, \zeta^t):=\frac{1}{\abs{\zeta^t}}\sum_{i\in \zeta^t}\nabla f_i(\theta_{t-1})$, where $\zeta^t$ is a minibatch sampled uniformly from the dataset $\{1, 2, \dots, n\}$. 

When training large neural networks, the dimensionality of $\theta$ is huge. Storing the model-related statistics, including the model $\theta$, the momentum $m$, and the gradient $\nabla \Tilde{f}(\theta)$ can be a major memory overhead. We call these statistics collectively as the \emph{model memory}. For example, the GPT-2~\citep{radford2019language} model has 1.5 billion parameters. During training, each parameter requires $32 \mathrm{(model)} + 32 \mathrm{(grad.)} + 32 \mathrm{(momentum)}$ bits or 12 bytes of model memory. Therefore, the model memory alone takes about $1.5\times 10^9 \times 12\mathrm{bytes}=17.6\mathrm{GB}$ of GPU memory, which already exceeds the capacity of many mainstream GPUs. 

To reduce training memory footprint, we can store the model-related statistics in low numerical precision. This involves a \emph{quantizer} $Q(\cdot)$, which encodes full-precision (32-bit) values to lower-precision ones, such as 8-bit integers. 
% Different statistics can be applied to different quantizers and we use different notations to avoid ambiguity.
The training procedure can be summarized as:
\begin{align}\label{eqn:lpmm}
g_t\leftarrow \quant{\nabla \Tilde{f}(\theta_{t-1})},~~~~
    m_{t}  \leftarrow \quant{\beta m_{t-1} + \nabla \Tilde{f}(\theta_{t-1})},~~~~
    \theta_{t}  \leftarrow \quant{\theta_{t-1} - \alpha m_t}.
\end{align}
Here, $g_t$ is a gradient accumulator, which stores the temporary gradients during back-propagation. 
When the parameters and momentum are updated, they are first decoded to full-precision, computed in full-precision, and then encoded and stored in low-precision, as illustrated in Fig.~\ref{fig:diagram}. We defer further implementation details to Sec.~\ref{sec:impl}.
% \jianfei{TODO: a diagram for illustration}

%we can apply a quantization function $Q(\cdot)$ to all model-related states including parameters, gradients, momentum and other possible optimizer states,
% to transfer the float point number into a low bit representation after all of computation in each iteration,
% such that they are persistent stored with less memory.
% When they are need again in the computation of the next iteration, the full-precision value is decoded from the low bit representation. 
% In other words, every operation except the storing is as usual.

\iffalse
Taking SGDM as an example, the training method introducing this kind of quantization is given by Algorithm \ref{alg:q-sgdm}. 


\begin{algorithm}
  \caption{Baisc Model Memory Quantized SGDM}
  \label{alg:q-sgdm}
  \begin{algorithmic}[1]
    \REQUIRE{initial parameter $\theta_0 \in \Rb^p$, learning rate $\alpha$, initial momentum $m_0 = 0 \in \Rb^p$, quantization function $Q$, total number of iterations $T$, momentum factor $\beta$}
    \FOR{$t = 1, 2, \dots, T$}
      \STATE Sample a minibatch $\zeta^t$ uniformly from the training data;
      \STATE $g_{t} \leftarrow Q(\nabla f(\theta_{t-1}, \zeta^t))$
      \STATE $m_{t} \leftarrow Q(\beta m_{t-1} + g_{t})$
      \STATE $\theta_{t} \leftarrow Q(\theta_{t-1} - \alpha m_t)$
    \ENDFOR
    \RETURN {$\theta_T$}
  \end{algorithmic}
\end{algorithm}
\fi

\subsection{The Underflow Problem}

% In order to really reduce the model memory, we need to guarantee lossless accuracy for our optimization framework.
% Unlike some previous work that found the major bottleneck results from quantization function or outliers,
% we discover that the main problem in our optimization framework is \emph{underflow}.
% To tell what \emph{underflow} indicates, we give some formal explanations.

Quantization is lossy, which can only represent values up to a numerical precision. Consider the following symmetric linear quantizer $Q = Q_{\delta, B}: \Rb \to \Rb$ as an example:
% We use standard linear symmetric quantization for simpler illustration and nonlinear quantization is also compatible in our analysis.
% Specifically, the quantization function 
\begin{align}
    \label{eq:q-def}
    Q_{\delta, B}(x) = \delta \cdot \text{Round}\left(\text{clip}\left(x/\delta, -B, B\right)\right),
\end{align}
where $\text{Round}(\cdot)$ is a rounding function and $\mathrm{clip}(\cdot, -B, B)$ clamps the input into the range $[-B, B]$. The quantizer $Q_{\delta, B}(x)$ converts $x$ to quantities within the range $[-\delta B, \delta B]$, up to the numerical precision $\delta$. The quantized value can be stored as a $\log_2(2B)$-bit integer. The quantizer can be generalized to vector inputs and outputs by applying element-wise to each entry. 

\emph{Arithmetic underflow} occurs when we try to sum up two quantities of different orders of magnitude. Consider the summation 
%where $\delta > 0$ is the \emph{quantization interval}, the representable number with minimal norm and $B$ is relevant to number of representable. 
\begin{align}
    \theta_{t} = Q_{\delta, B}\left(\theta_{t-1} + v_{t}\right),
\end{align}
where $\theta_t$ is the parameter at the $t$-th iteration, and $v_{t}=-\alpha m_{t}$ is the update vector.
Since $\theta_{t-1}$ itself is already in low-precision, we have $Q_{\delta, B}(\theta_{t-1})=\theta_{t-1}$.
Now, if the update is smaller than parameters' numerical precision, \ie~$\abs{v_{t, d}} < \delta / 2$ for some dimension $d$, the small update will be ``eaten'' by the large parameter, treated effectively as zero:
%then deterministic rounding function will output the value identical in the last iteration, i.e.
%computed in the $(t+1)$-th iteration. To get $\theta_{t+1}$, we perform
% \begin{align}
%     \theta_{t+1} = Q\left(\theta_t + v_{t+1}\right)
% \end{align}
%Note that $\theta_t$ is at the quantization point and $v_{t+1} = -\alpha m_{t+1}$ in SGDM algorithm. 
%As the training proceeds, the learning rate decays and the gradient norm becomes more flat, which both leads to smaller update vector. 
%Then \emph{underflow} occurs: if
\begin{align}
    \label{eq:eaten}
    \theta_{t, d} = Q_{\delta, B}\left(\theta_{t-1, d} + v_{t, d}\right) = \theta_{t-1, d}.
\end{align}
The update is likely to be small, particularly at the late stage of training where  the gradient (and momentum) is close to zero, and the learning rate is also decreased around zero. 
If underflowing occurs, the actual update direction $\tilde v_t:=\theta_{t}-\theta_{t-1}$ is far from the expected. the Extremely, there could be $\tilde v_t=0$, where the optimization completely stalls. %\jianfei{this paragraph still needs polishing}
%For full-precision optimizers, this is not a problem since the sum of many small updates can still be large. However, this underflowing problem is deadly for low-precision optimizers, since the optimization can completely stuck at some point. 

As shown in Fig.~\ref{fig:bin-change-ratio}, when the underflow problem is serious (fewer bits), the deterministic quantizer has the smallest actual update $\tilde v_t/\delta$. Actually, the deterministic quantizer hardly updates the parameters. 
As shown in Fig.~\ref{fig:proba-hist-mb1}, about 60\% entries in the update vector is less than $\delta / 2$. These entries are ignored by the deterministic quantizer.




\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/bin-change-ratio-12b8b8b-single-p.pdf}
        \caption{12-bit}
        \label{fig:12-bit-bin-change-ratio}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/bin-change-ratio-10b8b8b-single-p.pdf}
        \caption{10-bit}
        \label{fig:10-bit-bin-change-ratio}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/bin-change-ratio-8b8b8b-single-p.pdf}
        \caption{8-bit}
        \label{fig:8-bit-bin-change-ratio}
    \end{subfigure}
    \caption{The magnitude of parameter update for a convolution layer in ResNet-18. We vary the parameter precision from 12-bit to 8-bit.  Gradients and momentum are always in 8-bit. 
    The ``bin change ratio'' is defined as $\tilde v_t/\delta$ averaged over all dimensions. Larger is better. }%All these experiments run with a static quantization precision.}
    \label{fig:bin-change-ratio}
\end{figure}

\subsection{Solutions to the Underflow Problem}\label{sec:solutions}

We propose two methods for solving the underflow problem: unbiased stochastic quantization and gradient accumulation.

\paragraph{Unbiased Stochastic Quantization}
Stochastic quantization adopts an stochastic quantizer $Q(\cdot)$, satisfying $\E{Q(x)}=x$. 
A simplest stochastic quantizer is the following:
\begin{align}
    \label{eq:sq-def}
    Q_{\delta, B}(x) = \delta \cdot \text{SR}\left(\text{clip}\left(x/\delta, -B, B\right)\right),
\end{align}
where $\text{SR}(\cdot)$ is the stochastic rounding~\citep{gupta2015deep, courbariaux2015binaryconnect} operation:
\begin{align*}
\text{SR}(x)=
\ceil{x}  ~~\mbox{with probability } x-\floor{x} \mbox{otherwise} \floor{x}.
\end{align*}
The quantizer is unbiased as long as $\delta B \ge \abs{x}$. Stochastic quantization mitigates underflow by accumulating small updates in a probabilistic manner. When the update is small in magnitude, each dimension only has a small probability to be updated. Yet after a large number of updates, the final parameters still have the same expectation with the full-precision ones. Besides this informal argument, unbiased stochastic quantization is also the key to establish the convergence theory, as we shall see soon in Sec.~\ref{sec:convergence}. 

\iffalse
We point out unbiased stochastic quantization is critical for low bit training.
When the states are represented in a low bit format, the approximation error will increase greatly as the bits goes down.
Therefore, keeping the intrinsic property for quantized objects is more important than reducing the approximation error and one of the most critical property is the unbiasedness.

However, we need to figure out what unbiasedness stands for.
It is not referred to an stochastic quantization function with unbiasedness property, 
it means the unbiasedness of update vector under the randomness of all stochastic quantization.
In SGD with Momentum, since the update vector is linear to gradient and momentum, simple method like stochastic exactly satisfies the unbiasedness condition.
In our framework, we use the linear quantization defined as \ref{eq:q-def} and a nonlinear quantization technique proposed by \cite{dettmers20218}.
We observe the bad performance in the absence of unbiasedness experimentally. 
And our theoretical analysis is totally built on the unbiasdness condition.
\bingrui{Do we talk about what quantization function we used here? or in the `technique' section?}
\fi

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/proba-hist-8b8b8b-single-p-mb1-epoch9.pdf}
        \caption{Micro-batch size $N=1$}
        \label{fig:proba-hist-mb1}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/proba-hist-8b8b8b-single-p-mb8-epoch9.pdf}
        \caption{Micro-batch size $N=8$}
        \label{fig:proba-hist-mb8}
    \end{subfigure}
    \caption{The distribution of update vector magnitude across dimensions.  The result is counted at the epoch 10 for a single layer in ResNet-18. The blue bar (left Y-axis) represents the density and the red line (right Y-axis) indicates the cumulative distribution.} %These two experiments use different micro batch size $N$. 
    \label{fig:proba-hist}
\end{figure}

\paragraph{Microbatching}
% Gradient accumulation is a technique for enlarging learning rate and batch size without consuming more memory. 
% According to the convergence analysis for quantized SGD in previous work \cite{li2019dimension}, enlarging learning rate can improve the quantization error bound and get better stationary.

Underflowing arises from the difference in magnitude of the parameter and the update. Therefore, it can be mitigated by enlarging the update. \emph{Microbatching}~\citep{huang2019gpipe} works by summing up the gradient of multiple batches before applying the update to the momentum and parameters. More concretely, we can accumulate the gradient of $N$ mini-batches as
\begin{align*}
g_{t, 0}\leftarrow 0,~~~~g_{t, i} \leftarrow Q(g_{t, i-1} + \nabla f(\theta_{t-1}, \zeta^{t,i})),
\end{align*}
and use $g_{t, N}$ in place of $g_t$ for updating the momentum in Eq.~(\ref{eqn:lpmm}). Now, the accumulated gradient $g_{t, N}$ is $N$ times larger than the original $g_t$. Subsequently, the update $-\alpha m_t$ becomes $N$ times larger, yet the magnitude of the parameter $\theta_t$ is unchanged, so underflowing is significantly alleviated. 

As shown in Fig.~\ref{fig:proba-hist}(a), about  20\% entries of update vector $v_{t}$ are even smaller than ${\delta} / {8}$. 
In this case, vanilla stochastic quantizer can still suffer from high variance due to the repeated small updates. Microbatching significantly enlarge the size the update, and reduce the number of small updates (which underflow), as shown in Fig.~\ref{fig:proba-hist}(b). 

%However, we first point out that the underflow is possible to happen even if the stochastic rounding is adopted. 
%In our experiments on ResNet-18, we observed that nearly, as shown in . 
%Vanilla stochastic quantizer is useless for this case since the rounding probability $p \ll 1$.
%While the algorithm can do stochastic rounding again and again, it requires lots of rounding to take a leap and is therefore inefficient.
%We can see that over half of elements are less than $\delta / 2$ and nearly 20\% elements has a magnitude less than $\delta / 8$ in Fig.\ref{fig:proba-hist-mb1}. 

Micro-batching can be viewed equivalently as large-minibatch SGD~\citep{goyal2017accurate}, which simply multiply the batch size and the learning rate by $N$. Large-minibatch SGD is known to converge similarly to the original, small-minibatch SGD. However, enlarging the batch size is not memory efficient since the data memory will increase. 


% if there is a gradient $g$ at parameter $\theta$ indicating increasing with a quite small magnitude compared to the quantization interval, then the rounding probability $p = |g|/$
% stochastic rounding will probably ignore this tiny advance since the rounding probability is quite small. 
% And a leap cannot happen even if we quantize many times. 
% In this case, rounding with a bigger probability once is simpler than rounding with a small probability again and again.
% In fact, there are other reasons why the gradient accumulation can reduce the quantization error related to the magnitude of parameters, gradients and momentum buffers in the training process.
% We will analyze the convergence of these two algorithms and compare more formally in the next section.
%Theoretically, We later show that gradient accumulation not only plays a role like enlarging learning rate to reduce quantization error and reach better stationary but also has own advantages over it.
% without increasing other quantization error.
% Compared with enlarging learning rate simply, gradient accumulation has its own advantages in this setting.

% However, when we do gradient accumulation, gradients become persistent in the memory like parameters, which means it will consume the same amount of memory as parameters. 
% While in one-step update, gradient can be immediately accumulated into the momentum or parameter as soon as it is calculated.

% To solve this problem, we need to quantize the gradient like we quantize other states.
Putting it all together, we propose \method-SGDM, an optimizer with low-precision gradient accumulators, momentum, and parameters. The entire training procedure is given by Algorithm \ref{alg:q-sgdm-gc}. 
Fig.~\ref{fig:bin-change-ratio} and~\ref{fig:proba-hist} show that our algorithm effectively mitigate underflow with significantly larger updates. 

%our solution has larger ratio and make the distribution of update flatter compared with vanilla stochastic quantizer, which indicates that the underflowing is improvd.

%, while the stochastic quantizer can still update parameters with a small probability. 

% The stochastic quantizer  improves this situation. 
% And 
% , which are all ignored. 
% , then be ignored while  can keep going.

% Once the quantizer encounters this situation, it will be probably stuck in this point since the gradient is calculated at the same parameter and update vector still has the same magnitude.


\begin{algorithm}
  \caption{\method-SGDM}
  \label{alg:q-sgdm-gc}
  \begin{algorithmic}[1]
% \Procedure{Euclid}{$a,b$}\Comment{The g.c.d. of a and b}
    \REQUIRE{initial parameter $\theta_0 \in \Rb^p$, learning rate $\alpha$, initial momentum $m_0 = 0 \in \Rb^p$, quantization function $Q$, total number of iterations $T$, momentum factor $\beta$, gradient accumulation steps $N$}
    \FOR{$t = 1, 2, \dots, T$}
      \STATE $g_{t, 0} \leftarrow 0$
      \FOR{$i = 1, 2, \dots, N$}
      \STATE Sample a minibatch $\zeta^{t,i}$ uniformly from the training data;
      \STATE $g_{t, i} \leftarrow Q(g_{t, i-1} + \nabla f(\theta_{t-1}, \zeta^{t,i}))$
      \ENDFOR
      \STATE $m_{t} \leftarrow Q(\beta m_{t-1} + g_{t, N}))$
      \STATE $\theta_{t} \leftarrow Q(\theta_{t-1} - \alpha m_t)$
    \ENDFOR
    \RETURN {$\theta_T$}
% \EndProcedure  
  \end{algorithmic}
\end{algorithm}

\subsection{Informal Analysis}
We consider an SGD algorithm:
\begin{align*}
\theta_{t+NM}&\leftarrow \theta_t - \alpha \sum_{i=0}^{NM} \nabla f(\theta_t)\\
\end{align*}
In the \emph{linear learning rate scaling} regime, the optimization trajectory of the full-precision algorithm with different $N$ and $M$ stays close to each other (they discretize the same gradient flow).

Rewrite the iteration in the following 3-level accumulation form:
\begin{align*}
\theta_{t+NM}&\leftarrow Q(\theta_t - \alpha m_N)\\
m_{n+1}&\leftarrow Q(m_n + g_{nM})\\
g_{nm+1}&\leftarrow Q(g_{nm} + \nabla f_{t+nM+m}(\theta_{t}))
\end{align*}
We would like to know that: how to choose $N$ and $M$, so the variance of $\theta_T$ is minimized?

The problem is still somewhat too complicated, we can simplify the problem as follows:
\begin{align*}
\theta_{t+NM}&\leftarrow Q(\theta_t - \alpha m_N)\\
m_{n+1}&\leftarrow Q(m_n + g_{nM})\\
g_{nm+1}&\leftarrow Q(g_{nm} + \nabla f_{t+nM+m}(x_{t}))
\end{align*}
where $x_0, \dots, x_T$ is a fixed given sequence of parameters. 

Define $R(\theta)$ to be the numerical range of a vector. $R$ is a linear operator: $R(\alpha\theta) = \alpha R(\theta)$.

Assume that the range of $R(\theta_t)$ stays stationary...
\jianfei{I might be incorrect on the following quantization variance bounds}
\begin{align*}
\Var{Q(\theta_t - \alpha m_N) | \theta_t - \alpha m_N} &= 2^{-2a}R(\theta)^2 \\
\Var{Q(m_n + g_{nM}) | m_n + g_{nM}} &= 2^{-2b}R(m_N)^2 \\
\Var{Q(g_{nm} + \nabla f_{t+nM+m}(x_{t})) | g_{nm} + \nabla f_{t+nM+m}(x_{t})}
&= 2^{-2c}R(g_{nM})^2
\end{align*}
Further assume that $R(m_N) = \sqrt{N} R(m_1)$ 
and $R(m_1) = R(g_{0M}) = \sqrt{M} R(g_{01}) = \sqrt{M} R_g$
, we have
\begin{align*}
\Var{Q(\theta_t - \alpha m_N) | \theta_t - \alpha m_N} &= 2^{-2a}R_\theta^2 := V_\theta\\
\Var{Q(m_n + g_{nM}) | m_n + g_{nM}} &=  2^{-2b}NM R_g^2 := V_m \\
\Var{Q(g_{nm} + \nabla f_{t+nM+m}(x_{t})) | g_{nm} + \nabla f_{t+nM+m}(x_{t})}
&= 2^{-2c}M R_g^2  := V_g
\end{align*}


Then, by law of total variance we have 
\begin{align*}
\forall n, \Var{g_{nM}} &= 2^{-2c} M^2 R_g^2 \\
\forall n, \Var{m_n} &= n V_m + \sum_{i=0}^{n-1} \Var{g_{i}m}
= n V_m + n 2^{-2c} M^2 R_g^2 = n R_g^2 (2^{-2b} NM + 2^{-2c} M^2). \\
\Var{m_N}&= R_g^2 (2^{-2b} N^2M + 2^{-2c} N M^2)\\
\Var{\theta_{t+NM}} &= \E{\Var{\theta_{t+NM} | \theta_t - \alpha m_N}}
\end{align*}

Therefore, we have
\begin{align*}
\Var{\theta_T} \approx 2^{-2a}\frac{T}{NM} R_\theta^2 + \left(2^{-2b}TN^2M + 2^{-2c}TM^2\right)R_g^2.
\end{align*}

The question is, given a bit-budget $d$, how can we determine $a, b, c$ and $N, M$ to minimize the variance?
\begin{align*}
\min_{a,b,c,N,M}&  \Vc := 2^{-2a}\frac{T}{NM} R_\theta^2 + \left(2^{-2b}TN^2M + 2^{-2c}TM^2\right)R_g^2\\
\mbox{s.t.} & a+b+c=d
\end{align*}

This might be hard. Consider a special case where $N=1$ and $a, b, c$ are given. Then the momentum quantization variance is zero. We have 
\begin{align*}
\Vc^\prime M \propto -V_\theta M^{-2} + 2 V_g M = 0,
\end{align*}
\bingrui{1. Why does the momentum quantization variance become zero when N = 1? 2. Here might be $\Vc/M$?}\jianfei{we do not need to store the momentum anymore}\bingrui{But we need to store the momentum over time no matter the N?}
\jianfei{anyway, this special case is not really of much interest.}\bingrui{fine}

so the minimum $M^* = \left(\frac{V_\theta}{2V_g}\right)^{1/3}$ and 
$\Vc^* \propto T V_\theta ^{2/3} V_g^{1/3} $. On the other hand, when $M=1$, we have $\Vc^* \propto T V_\theta + 2TV_g\approx TV_\theta$, which is $\left(\frac{V_\theta}{V_g}\right)^{1/3}$ times worse. 

\paragraph{Remark: } If $T\alpha$ is a constant, this also directly shows that larger $\alpha$ is better, since the variance is proportional with $T$ (inversely proportional with $\alpha$). 
\bingrui{On the other hand, the gradient variance from SGD arises as $\alpha$ gets larger}
\paragraph{Remark: } In case of $M=1$ and $V_\theta \gg V_g$. Increasing $M$ by two times implies that we can decrease the (parameter quantization variance) by four times, in this case, we can safely reduce the bitwidth of parameter by 1. 

For the general problem, my hunch is that we should choose the hyperparameters so that the three variance terms are equal.\jianfei{maybe my hunch is wrong. Try directly solve with Langrange multipliers?} (Note that the problem should not be too hard since the solution only depend on $\rho$ and $d$.)
Suppose $N, M$ are given, we have 
$2^{-2a}\frac{T}{NM} R_\theta^2 =  2^{-2b}TN^2M R_g^2 = 2^{-2c}TM^2 R_g^2$. Define $\rho = R_\theta / R_g$, we have 
\begin{align*}
    2^{-2a} \frac{1}{NM} \rho^2 = 2^{-2b} N^2 M = 2^{-2c} M^2.
\end{align*}
or
\begin{align*}
a - \log_2 \rho + \frac{1}{2}\log_2 N + \frac{1}{2}\log_2 M  = b - \log_2 N - \frac{1}{2}\log_2 M = c - \log_2 M.
\end{align*}
(If $N=M=1$, this means that $a-\log_2 \rho = b = c$.)
\bingrui{When $N=1, M>1$(which is the just microbatching setting), we need more bits for gradient (i.e.~$c$) compared with momentum from this equation. However the experiments tell us the gradient is more tolerant to lower bits when momentum exists.}
Given that $a+b+c=d$,we have 
\begin{align*}
    a &= \frac{1}{3}d + \frac{2}{3}\log_2 \rho - \frac{2}{3}\log_2 N -\frac{5}{6}M \\
    b &= \frac{1}{3}d - \frac{1}{3}\log_2 \rho + \frac{5}{6}\log_2 N +\frac{1}{6}M \\
    c &= \frac{1}{3}d - \frac{1}{3}\log_2 \rho - \frac{1}{6}\log_2 N +\frac{2}{3}M \\
\end{align*}
In this case,
\begin{align*}
    \Vc^* = 3\times 2^{-\frac{2}{3}d}\rho^{\frac{2}{3}} N^{\frac{1}{3}} M^{\frac{2}{3}}.
\end{align*}
It appears that increasing $N$ and $M$ monotonically make things worse......?!


\paragraph{Try again: Lagrange multiplier}
Define $\Lc = 2^{-2a}\frac{1}{NM} \rho^2 + 2^{-2b}N^2M + 2^{-2c}M^2 + \lambda (a+b+c-d).$ We have
\begin{align*}
-2a \ln 2\times 2^{-2a}\frac{1}{NM} \rho^2 + \lambda &= 0 \\ 
-2b \ln 2\times 2^{-2b}N^2M + \lambda &= 0 \\ 
-2c \ln 2\times 2^{-2c}M^2 + \lambda &= 0 \\
a+b+c&=d.
\end{align*}
It cannot be directly solved, but I think the result would be similar... Why?
\jianfei{Checked with numerical results. Indeed, larger $N, M$ is worse. Maybe the variance model is wrong?}
\iffalse
while the quanse
\subsectization) ion{}


\jianfei{we can consider the simplified setting: computing $\sum_{t=1}^T v_t$}
% \jianfei{maybe also discuss the 3-layer summation here...}

Intuitively, we can use the value of rounding probability to give an interpretation about the role of gradient accumulation in a simple 1-d case.
Suppose we use stochastic rounding quantization and take gradient descent at parameter $\theta$. The gradient at this point is $g$ and step size is $\alpha$, thus the update vector is given by $v = -\alpha g$.
Experimentally, we can always observe that the update vector has a quite small magnitude compared to the quantization interval $\delta$. 
Since $\theta$ is at one quantization point, the rounding probability can be written as $p = \abs{\alpha g} / \delta$.
If we use the gradient accumulation with $N$ micro batches, then this probability is expanded by $N$ times.
Rounding with $N$ times the probability once is much better than rounding $N$ times with the original probability since for fixed $N$ we always have
\begin{align}
    1 - (1-p)^N \le Np,\, \forall p \in [0, 1]
\end{align}

\jianfei{make the insight clear: tradeoff the underflow error of $g$ with $\theta$.}


\fi

\subsection{Exact microbatching}
Consider the Momentum SGD updates:
\begin{align*}
\theta_{t}=\theta_{t-1} - \alpha m_t, m_{t} = \beta m_{t-1} + g_{t}.
\end{align*}
Equivalently, let's do the following updates:
\begin{align*}
\forall i\in [1, N], s_{t+i} = \sum_{j=1}^i m_{t_0+j},
\theta_{t_0+N}=\theta_{t_0} - \alpha s_{t_0+N}.
\end{align*}
Moreover, define
\begin{align*}
\forall i\in [1, N], p_{t_0+i} = m_{t_0+1} + \sum_{j=2}^{i}g_{t_0+j} 
\end{align*}
We have
\begin{align*}
\forall i\in [1, N),
s_{t_0+i+1} &= m_{t_0+1} + \sum_{j=1}^{i} m_{t_0+j+1}
= m_{t_0+1} + \sum_{j=1}^{i} (\beta m_{t_0+j} + g_{t_0+j+1} )\\
&= \beta s_{t_0+i} + m_{t_0+1} + \sum_{j=2}^{i+1}g_{t_0+j}  \\
&= \beta s_{t_0+i} + p_{t_0+i+1}
\end{align*}

Given $t_0$, we can keep the follow up states as $(\theta_{t_0}, s_{t_0+i}, p_{t_0+i})$ rather than $(\theta_{t_0+i}, m_{t_0+i}, g_{t_0+i})$. 

\begin{enumerate}
\item $\forall i\in (2, N]$, we can update
\begin{align*}
p_{t_0+i} = p_{t_0+i-1} + g_{t_i+i},
~~~~s_{t_0+i} = \beta s_{t_0+i-1} + p_{t_0+i}.
\end{align*}
\item If $i=N$, we should update 
\begin{align*}
\theta_{t_0+N} = \theta_{t_0} - \alpha s_{t_0+N}
\end{align*}
then, we should prepare the next $s_{t_0+N+1} = p_{t_0+N+1} = m_{t_0+N+1}$. Note that 
\begin{align*}
m_{t_0+N+1} = s_{t_0+N+1} - s_{t_0+N} = (\beta - 1)s_{t_0+N} + p_{t_0+N+1} = (\beta - 1)s_{t_0+N} + p_{t_0+N} + g_{t_0+N+1}.
\end{align*}
Therefore, we can set
\begin{align*}
s_{t_0+N}\leftarrow (\beta-1)s_{t_0+N} + p_{t_0+N},~~~~
p_{t_0+N}=\mbox{anything}.
\end{align*}
\item Finally, when $i=1$, we can update
\begin{align*}
p_{t_0+1} = s_{t_0+1} = s_{t_0} + g_{t_0+1}.
\end{align*}

\paragraph{Remark 1: }
For Adam, I guess that simply using a stale version of the second order momentum will work. I.e., whatever we require $\theta_t$, we compute $\theta_{t_0} - \alpha s_t / (\sqrt{v_t} + \epsilon)$. The reason is that $v_t$ changes very slowly anyway $(\beta_2=0.999)$.

\paragraph{Remark 2: }
If we quantize the gradient, the problem is the same: this ``microbatching'' still increases the required bitwidth of the gradient. 

\paragraph{Remark 3: } $p$ is stored in the gradient accumulation buffer. For DDP, we do \texttt{allreduce} to $p$ instead of $g$. But this is equivalent in the full-precision scenario. 

\end{enumerate}


==> src/4-convergence.tex <==
In this section, we analyze the convergence of the proposed \method-SGDM algorithm and discuss the impact of the proposed techniques. 
%give the convergence analysis of Quantized SGDM (Algorithm \ref{alg:q-sgdm}) and Quantized SGDM with Gradient Accumulation (Algorithm \ref{alg:q-sgdm-gc}), which is not given in previous analysis. 

\subsection{Assumptions}
First, we make some assumptions. The first three are rather standard in stochastic optimization literature, while last two depict properties of  stochastic quantizers. 

%\paragraph{Assumptions}
\emph{
\begin{myitems}
    \item (Convexity) The objective function is convex and has an unique global minimum $f(\theta^*)$.
    \item (Smoothness) The objective $f(\theta)$ is continuous differentiable and $L$-smooth;
    % i.e. $f(y) - f(x) \le \langle \nabla f(x), y - x \rangle + \frac{L}{2}\norm{x - y}^2$
    \item (Bounded variance) $ \Eb\left[\norm{\nabla\Tilde{f}(\theta) - \nabla f(\theta)}^2\right] < \sigma^2$, $\forall \theta \in \mathbb{R}^d$.
    \item (Unbiased quantizer)  $\forall x\in \mathbb R^d$, $\E{Q_p(x)}=\E{Q_g(x)}=\E{Q_m(x)}=x$.
\item (Bounded quantization variance) $\forall x\in \mathbb R^d$, $\E{\norm{Q_p(x)-x}^2}\le \sigma_p^2$,
$\E{\norm{Q_g(x)-x}^2}\le \sigma_g^2$,
$\E{\norm{Q_m(x)-x}^2}\le \sigma_m^2$.
\end{myitems}
}

Here, Assumption 3 depicts the variance of sampling mini-batches, and Assumption 5 bounds quantization error of model-related statistics through the variance. 
Assumptions~4-5 can be realized by the linear quantizer in Eq.~(\ref{eq:sq-def}), where we have $\E{\norm{Q_{\delta, B}(x) - x}^2}\le \frac{\delta^2 d}{4}, \forall x\in \mathbb R^d$.%~\citep{?}. 
Yet, our analysis is applicable to other non-linear quantizers such as those discussed in Sec.~\ref{sec:nonlinear-quantization}.
We assume that the objective function is convex, which is somewhat restrictive. 
However, this simple convex case is sufficient to reflect the underflowing challenge of training with low-precision model memory, and we leave the non-convex case as a future study. 

\iffalse
There are many choices to define the quantization function, and different quantization functions can be applied to different variables and at different iterations.
Here we use the standard symmetric linear quantization, denoted by $Q(\cdot)$, to analyze the quantization error. Formally, suppose we quantize a 32-bits full precision vector $x \in \mathbb{R}^d$ into a format where each element $x_i$ is represented by $b$ bits. 
Let $B$ be the maximal integer representable. For signed case, we often have $B = 2^{b-1} - 1$.
Then we have $Q(\cdot)$ of the form
\begin{align}
    % \label{eq:q-def}
    Q(x)_i = \frac{\norm{x}_{\infty}}{B} \text{SR}\left(\frac{Bx_i}{\norm{x}_{\infty}}\right) 
\end{align}
where the SR denotes stochastic rounding. This quantization function has many nice properties, the most important one of which is the unbiasedness
\begin{align}
    \Eb[Q(x)] = x,\, \forall x \in \mathbb{R}^d
\end{align}

For the quantization error bound, we have 
\begin{align}
    \Eb[\norm{Q(x) - x}^2] \le \frac{\delta^2d}{4}
\end{align}
where $\delta$ is the minimal quantization interval. For the above quantization function, $\delta = \frac{\norm{x}_\infty}{B}$. Note that in the quantization of parameter, gradient and momentum, this $\delta$ is different.
Actually, the the unbiasedness of quantization is critical in our analysis and if we have other unbiased quantization with smaller quantization variance, the analysis can still holds with a more tight conclusion.
\fi

\subsection{Convergence of \method-SGDM}\label{sec:convergence}
%Let us do some preparations for quantized SGDM. 
We first analyze the bias and variance of the quantized gradient accumulator.

\begin{lemma}
    In Algorithm \ref{alg:q-sgdm-gc}, with Assumptions 3-5, the  first and second momentum of $g_{t,i}$ satisfy
    \begin{align}
        \Eb[g_{t, i} | \theta_{t-1}] & = i \nabla f(\theta_{t-1}) \\
        \Eb[\norm{g_{t, i}}^2 | \theta_{t-1}] & \le i\sigma_g^2 + i(i+2)\norm{\nabla f(\theta_{t-1})}^2 + i \sigma^2.
    \end{align}
\end{lemma}

Next, we construct an auxiliary sequence $\{z_t\}$, following previous analysis of heavy ball methods~\citep{ghadimi2015global} and SGDM~\citep{liu2020improved}:
%In [TODO:ref],  designed for the analysis of deterministic heavy ball methods is defined as 
\begin{align}
    \label{eq:zt-def}
    z_t = \theta_0, \text{when}~t = 0,~\text{otherwise}~
    \frac{1}{1 - \beta}\theta_t - \frac{\beta}{1 - \beta}\theta_{t-1}.
\end{align}
% Afterwards, it also applied in the analysis of SGDM in [TODO:ref]. 
The sequence enjoys the following nice properties:

\iffalse
\begin{lemma}
    Let $\delta_p$ and $\delta_m$ be the minimal quantization interval of parameters and momentum respectively.
    The sequences ${z_t}$ defined in \ref{eq:zt-def} satisfies
    \begin{align}
    z_{t+1} - z_{t} & = \frac{1}{1 - \beta} (\theta_{t+1} - \theta_t) - \frac{\beta}{1 - \beta}(\theta_t - \theta_{t-1}) \\
    \Eb[z_{t+1} - z_{t}] & = \frac{-\alpha}{1 - \beta} \nabla f(\theta_t) \\
    \Eb[\norm{z_{t+1} - z_{t}}^2] 
    & \le  \left(\frac{\alpha}{1-\beta}\right)^2 \left( \Eb[\norm{\nabla f(\theta_t)}^2] + \sigma^2 \right)
    + \left(\frac{\alpha}{1-\beta}\right)^2\frac{\delta_m^2d}{4}  + \frac{1 + \beta^2}{(1 - \beta)^2} \frac{\delta_p^2d}{4}
\end{align}
\end{lemma}
\jianfei{why do we want to upper bound (8)? Does this Lemma alone give any insight?}
Note that the quantity $\Eb[\norm{z_{t+1} - z_{t}}^2]$ can be composed by three parts: the variance of stochastic gradient, momentum quantization and parameter quantization error. 
Therefore, our analysis also give convergence for the algorithm when you choose not to quantize some training states since their variances are independent from each other.
With this lemma, we have following theorem characterizing the convergence of quantized SGDM.
\begin{theorem}
    \label{thm:q-sgdm}
    Consider the Algorithm \ref{alg:q-sgdm}. Let Assumption \ref{assump:stochastic-optim} hold and assume that $f$ is convex. Let the quantization be defined as \ref{eq:q-def}. Suppose that $\theta_*$ is an optimal parameter and $f_* = f(\theta_*)$ is the optimal objective value. Let $\alpha \in (0, \frac{1-\beta}{L}]$, then for all $T > 0$ we have
    \begin{align*}
        \Eb[f(\Bar{{\theta}}_T) - f_*] & \le \frac{1}{2T}\left( \frac{L\beta}{1-\beta} + \frac{1-\beta}{\alpha} \right) \norm{\theta_0 - \theta_*}^2\\
    & + \frac{\alpha \sigma^2}{2(1-\beta)} + \frac{\alpha\delta_m^2d}{8(1-\beta)}
    + \frac{(1+\beta^2)\delta_p^2d}{8\alpha(1-\beta)}
    \end{align*}
    where $\Bar{\theta}_T = \frac{1}{T}\sum_{i=0}^{T-1}\theta_i$ 
    % and $\delta_p$ and $\delta_m$ is the minimal quantization interval of parameters and momentum respectively.
\end{theorem}

\jianfei{so we assume unique global optimum without strong convexity? this looks somewhat unconventional}\jianfei{what about the result for sgd? Is it simply $\beta=0$?}
\jianfei{as $\beta\rightarrow 1$, both quantization variance term increases?}
\fi

\iffalse
\subsection{Convergence of Quantized SGDM with Gradient Accumulation}
Compared with Algorithm \ref{alg:q-sgdm}, Quantized SGDM with Gradient Accumulation also quantize the gradient accumulator.
Therefore we first state the following observation about the stochastic quantized gradient.

\begin{lemma}
    In Algorithm \ref{alg:q-sgdm-gc}, The conditional first and second momentum of $g_{t,i}$ satisfis
    \begin{align}
        \Eb[g_{t, i} | \theta_{t-1}] & = i \nabla f(\theta_{t-1}) \\
        \Eb[\norm{g_{t, i}}^2 | \theta_{t-1}] & \le \frac{i\delta_g^2d}{4} + i(i+2)\norm{\nabla f(\theta_{t-1})}^2 + i \sigma^2
    \end{align}
\end{lemma}
\fi 
%Since the algorithm changes, the property of $z_t$ also changes. We write the following lemma to talk about the property of $z_t$ in Algorithm \ref{alg:q-sgdm-gc}.
\begin{lemma}
If Assumptions 3-5 hold, then sequence $\{z_t\}$ satisfies
    %Let $\delta_p$, $\delta_g$ and $\delta_m$ be the minimal quantization interval of parameters gradient, and momentum respectively.
    %The 
    \begin{align}
        % z_{t+1} - z_{t} & = \frac{1}{1 - \beta} (\theta_{t+1} - \theta_t) - \frac{\beta}{1 - \beta}(\theta_t - \theta_{t-1}) \\
        % \Eb[z_{t+1} - z_{t}] & = \frac{-\alpha}{1 - \beta} \nabla f(\theta_t) \\
        % \Eb[\norm{z_{t+1} - z_{t}}^2] 
        % & \le  \left(\frac{\alpha}{1-\beta}\right)^2 \left( \Eb[\norm{\nabla f(\theta_t)}^2] + \sigma^2 + \sigma_m^2 \right) + \frac{1 + \beta^2}{(1 - \beta)^2} \sigma_p^2.
        z_{t+1} - z_{t} & = \frac{1}{1 - \beta} (\theta_{t+1} - \theta_t) - \frac{\beta}{1 - \beta}(\theta_t - \theta_{t-1}) \\
        \Eb[z_{t+1} - z_{t}] & = \frac{-\alpha N}{1 - \beta} \nabla f(\theta_t) \\
        \Eb[\norm{z_{t+1} - z_{t}}^2] 
        & \le  \left(\frac{\alpha}{1-\beta}\right)^2 \left( 2\Eb[\norm{g_{t+1,N}}^2] + \sigma_m^2  \right) + \frac{1 + 2\beta^2}{(1 - \beta)^2} \sigma_p^2.
    \end{align}
\end{lemma}

The quantity $\Eb[\norm{z_{t+1} - z_{t}}^2]$ is composed of four parts: the batch gradient norm, the variance of stochastic gradient, momentum quantization and parameter quantization error. 
The latter three noise terms sum up independently. 
Our analysis applies to cases when only some of the model-related statistics are quantized by setting corresponding noise terms to zero. 
With this lemma, we derive the following theorem characterizing the convergence of \method-SGDM.

%With these preparations, we immediately have the following theorem about convergence of Quantized SGDM with Gradient Accumulation.
\begin{theorem}
    \label{thm:q-sgdm-gc}
    Consider the Algorithm \ref{alg:q-sgdm-gc} with Assumptions 1-5.  Let $\alpha \in (0, \frac{1-\beta}{(N+2)L}]$, then for all $T > 0$ we have
    \begin{align}
    \Eb[f(\Bar{{\theta}}_T) - f_*] & \le \frac{1}{2T}\left( \frac{L\beta}{1-\beta} + \frac{1-\beta}{\alpha N} \right) \norm{\theta_0 - \theta_*}^2\\
    & + \frac{\alpha \sigma^2}{(1-\beta)} 
    + \frac{\alpha\sigma_g^2}{(1-\beta)}
    + \frac{\alpha\sigma_m^2}{2N(1-\beta)}
    + \frac{(1+2\beta^2)\sigma_p^2}{2\alpha N(1-\beta)}.\label{eqn:convergence-rate}
    \end{align}
    where $\Bar{\theta}_T = \frac{1}{T}\sum_{i=0}^{T-1}\theta_i$.
\end{theorem}

Theorem~\ref{thm:q-sgdm-gc} reveals the effectiveness of the proposed techniques in Sec.~\ref{sec:solutions}. 
First, \method~can converge to the global optimum when $T\rightarrow \infty$, $\alpha\rightarrow 0$, and $\alpha N\rightarrow \infty$ for any quantizer with non-zero $\sigma_p$, $\sigma_g$, and $\sigma_m$. That is, the ultimate convergence is guaranteed regardless of the numerical precision. In contrast, optimizers with deterministic quantizers could stall at some intermediate state, as discussed in Sec.~\ref{sec:solutions}. Therefore, stochastic quantization is essential for the convergence guarantee. 


Second, we can study the impact of gradient accumulation.
With sufficiently large $T$, the first term in Eq.~(\ref{eqn:convergence-rate}) vanishes, and we therefore only consider the noise terms. 
We compare a plain algorithm ($N=1$) and a version with gradient accumulation ($N>1$), with equal learning rate. 
Gradient accumulation reduces the parameter quantization error (the $\sigma_p$ term) by $N$ times. Meanwhile, the gradient accumulator stores the  gradient sum over $N$ mini-batches, so $\sigma_g$ becomes larger. 
Therefore, gradient accumulation trades gradient quantization error for parameter quantization error. 
The error bound is tighter with a large $N$ when parameter quantization error is more significant, which holds true according to our empirical observations in Fig.~\ref{fig:bin-change-ratio} and \ref{fig:proba-hist}.
% \bingrui{TODO}

%. Actually, in our empirical observations, the magnitude of gradients is smaller than the parameters at most times thus this condition holds.

% Given a learning rate $\alpha$
% For Algorithm \ref{alg:q-sgdm-gc}, the quantization errors of parameters and momentum are reduced by $\frac{1}{N}$  and the gradient quantization error is introduced.

%This reflects the effectiveness of stochastic quantization. 

% This reflects the effectiveness of stochastic quantization, since 

% The effectiveness of stochastic quantization 

%According to Theorem \ref{thm:q-sgdm}, one of the easiest and straightforward approach is to increase the learning rate. However, this raises two problems. First, the size of minibatch has to be linearly increased in order to adapt to the increased learning rate. 
% Second, from the bound in theorem, the quantization error from momentum cannot be improved by simply increasing the learning rate. 
% Next, we are going to show that all kinds of quantization error can be improved by applying gradient accumulation.


% Here we compare the results given by Theorem \ref{thm:q-sgdm-gc} with Theorem \ref{thm:q-sgdm} for the convex objective case.
% When the two algorithms have equal learning rate, the stationary caused by stochastic gradient is identical, while the quantization errors of different terms vary. For Algorithm \ref{alg:q-sgdm-gc}, the quantization errors of parameters and momentum are reduced by $\frac{1}{N}$  and the gradient quantization error is introduced.
% Therefore, we will obtain a tighter bound of error bound when the reduced quantization error is more significant than the newly introduced error. Actually, in our empirical observations, the magnitude of gradients is smaller than the parameters at most times thus this condition holds.
\iffalse
On the other hand, the range of valuable learning rate of Algorithm \ref{alg:q-sgdm} is $N$ times more than Algorithm \ref{alg:q-sgdm-gc} and we can compare them when the learning rate taken in Algorithm \ref{alg:q-sgdm} is $N$ times that in Algorithm \ref{alg:q-sgdm-gc}. In this case, they have equal parameters quantization error while the momentum quantization error in Algorithm \ref{alg:q-sgdm} is enlarged $N$ times. 
And there still exists a trade-off which says that if the magnitude of gradients is smaller than the momentum buffers the total quantization error of the algorithm with gradient accumulation is smaller.
\jianfei{TODO}
\fi

==> src/5-technique.tex <==

In this section, we discuss our quantizer design and the implementation of the whole training framework.

\iffalse
\subsection{Unbiased Quantization}
\jianfei{do we still need this subsection?}
Formally, for a stateful optimizer, given the optimizer state $s_{t-1}$ in previous iteration $t-1$ and the minibatch sampling $\zeta^t$ in current iteration $t$, suppose that $v_t$ is the update vector induced by the original optimizer and $\hat{v}_t$ is the update vector induced by the quantized optimizer, the general unbiasedness guarantee is given by
\begin{align}
    \Eb[\hat{v}_t | s_{t-1}, \zeta^t] = v_t
\end{align}
Next, we will analyze the SGDM and Adam by substituting their specific optimizer states respectively.

\paragraph{SGDM}
For SGDM, we just use the traditional stochastic rounding in the quantization of momentum buffer. 
Based on this, the unbiasedness guarantee holds by
\begin{align}
    \Eb[m_t | m_{t-1}, \zeta^t] = \beta m_{t-1} + g_t
\end{align}

\paragraph{Adam}
Adam is a stateful optimizer with first momentum $m_t$ and non-negative second momentum $r_t$. 
Following its update rule, the update vector is linear to first momentum but nonlinear to second momentum.
Here we propose a pre-quantization transformation on the second momentum to guarantee the unbiasedness
\begin{align}
    r_t = T_2\left(Q\left(T_1\left(\beta_2 r_{t-1} + (1 - \beta_2) g_t^2\right)\right)\right)
\end{align}
where $T_1 = \frac{1}{\sqrt{\cdot}}, T_2 = \frac{1}{(\cdot)^2}$ element-wise.
And in the network training, we store the output by quantization function for memory saving. 
After applying this transformation, we can verify that
\begin{align}
    \Eb\left[\frac{m_t}{\sqrt{r_t}} | m_{t-1}, r_{t-1}, \zeta^t \right] = \frac{\beta_1 m_{t-1} + (1-\beta_1)g_t}{\sqrt{\beta_2 r_{t-1} + (1 - \beta_2) g_t^2}}
\end{align}
\fi


\subsection{Group and Nonlinear Quantization}\label{sec:nonlinear-quantization}
For the quantizer, we use the nonlinear quantization on momentum and linear quantization on parameters and gradients. 
All quantizers use the standard absmax symmetric quantization.
The linear quantization is defined as Eq.~\ref{eq:sq-def}. 
The nonlinear quantization method \citep{dettmers20158} proposes a novel floating-point  format in which the bitwidth for the exponent is dynamic.
Furthermore, given a tensor to be quantized, we first use the absmax to normalize the tensor into $[-1, 1]$. Then, the quantizer finds the bucket for each element with a binary search on a precomputed quantization map. Finally, the quantizer projects the value to one of the adjacent quantization points by stochastic rounding. Since stochastic rounding is unbiased, this nonlinear quantization method is also unbiased, which indicates that all the analysis above holds except the quantization variance is intrinsically different.

Group quantization is also adopted to avoid the negative impact of outliers. 
We chunk every tensor into groups of size 2048, and every group has its own quantization precision $\delta$.
However, group quantization introduces more data to be stored and as group size decreases, the quantization is more accurate while the extra data cost will be higher. We choose the group size of 2048 to balance the numerical precision and storage cost. 

\subsection{Dynamic Quantization}\label{sec:dynamic-quantization}
We experimentally observed that the magnitude of parameters shows a trend of first increasing and then decreasing. 
If a smaller quantization granularity $\delta$ is adopted, then the \emph{overflow} problems occur.
Especially at the initial stage of optimization, the quantizer rudely truncated the parameters to be increased due to limited range, which leads to a biased quantizer and makes the solution suboptimal. 
However, if we quantize with an overly large $\delta$, it results in poor numerical precision, and the underflow problem worsens.
Therefore, we take a dynamic quantization policy to balance the overflow and underflow.
Specifically, it calculates the quantization precision $\delta$ with the quantizers' inputs at every iteration, 
which gives a minimal lossless $\delta$. 
% \subsection{Adaptive Requantization}
% We use the adaptive requantization trick for stable training.
% If the quantizer normalizes the tensor using current absmax at every iteration, there is a requantization error since the minimal quantization interval changes all the time. 
% To reduce the impact of requantization error and let the network learn without confusion, we fix the quantization arguments every few dozen iterations and update them adaptively by the current tensor value.
% This will not only make network learning easy under a fixed quantization pattern, but also the quantized tensors can have a larger range of values.

\subsection{System Implementation}\label{sec:impl}
Here we discuss how our algorithm is implemented.
As illustrated in Fig.~\ref{fig:diagram}, the forward, backward, and optimizer steps are all depicted straightforwardly.
Before an iteration begins, we store all model memory in low precision.
When the new input comes, the parameters needed for forward computation are dequantized into a temporary full-precision ``copy''. Note that the parameters for each layer are not required simutaenously, so we only dequantize parameters right before its usage. 
As long as the computation related to the full-precision ``copy'' has finished, we delete these tensors. Therefore, the overhead of the temporary full-precision parameter is no larger than the largest single parameter tensor. 
In the backpropagation and optimizer step, a similar computation pattern happens.
Note that the memory of gradient accumulators cannot be saved by not storing the gradient accumulator even if we do not apply microbatching (\ie~$N=1$).
On the one hand, the gradient may not be calculated in one operation (or one layer). 
On the other hand, gradient computation can be composed of multiple accumulations, such as in a convolution layer.

Since the computation in neural network training is always layerwise, then at most, only the full-precision parameters, gradients, and momentum associated with one single layer are kept in memory at the same time, 
while other model memory is inactive and in low-precision.

Based on this philosophy, we implemented a training algorithm on PyTorch. 
We quantize the full-precision to low-precision representation by manually compressing them into a byte stream using the CUDA kernel.
Our system includes a lot of operators and layers to perform desired forward and backward calculations. 
Given a defined model, we quantize the parameter tensor individually, replace the original full-precision parameter and then move to GPU.
Then it can convert the layers of the model automatically by our customized layer. 
Besides, to get the gradient and perform computation more conveniently, we manually design a gradient accumulator instead of using the original ``grad'' attribute.



==> src/a2-addi-exp.tex <==



\section{Additional Experiments [TODO]}

\subsection{\textcolor{blue}{Experiment: ResNet Image Classification}}

Table~\ref{tab:resnet-quant-type-ablation} shows the effect of quantization methods on accuracy for ResNet-50 with SGD.

\begin{table}[h]
    \centering
    \caption{\textcolor{blue}{Effect of quantization methods on performance of ResNet-50 with SGD optimizer. We mainly focus on 4-bit momentum. One run.}
    }
    \label{tab:resnet-quant-type-ablation}
    \begin{tabular}{llc}
        \toprule
        Setting         & Method & top-1 acc. \\
        \midrule
        Ref.   & - & 77.1 \\
        \midrule
        FP32   & - & 77.2 \\
        8-bit Momentum & group & TODO \\
        4-bit Momentum & tensor & 76.0 \\
        4-bit Momentum & group  & 76.6 \\
        4-bit Momentum & dim0   & 76.7 \\
        4-bit Momentum & dim1   & 76.6 \\
        4-bit Momentum & rank-1 & 76.8 \\
        5-bit Momentum & rank-1 & 76.9 \\
        \bottomrule
    \end{tabular}
\end{table}

\subsection{\textcolor{blue}{Experiment: RoBERTa Finetuning}}

Table~\ref{tab:glue-accuracy} shows the results of RoBERTa-Large~\citep{liu2019roberta} finetuning on GLUE~\citep{wang2018glue} dataset. 
Each column is the median performance metrics (accuracy, F1, etc.) across 5 random seeds.
Similar to \method-SGDM, the \method-Adam adopt linear quantization on parameters and gradients, nonlinear quantization on momentum and square momentum.
The results show that consistent 8-bit \method-Adam could achieve (nearly) lossless 
accuracy compared with full-precision reference.

Table~\ref{tab:roberta-quant-type-ablation} shows the effect of quantization methods on accuracy for RoBERTa-Large finetuning with Adam.
For second moment, we also compare with sublinear memory methods including Adafactor~\citep{shazeer2018adafactor} and SM3~\citep{anil2019memory}. For fairness, we only add the memory efficient technique directly to Adam, while other techniques like no momentum and adaptive clipping are not applied. 
For this task, sublinear memory method is better in the sense of memory and accuracy trade-off.

\begin{table}[htbp]
    \centering
    \caption{Performance of RoBERTa-Large on GLUE Tasks. \method(12/8/8/8) means that 12-bit parameter, 8-bit gradient, 8-bit momentum, 8-bit second order momentum are used.
    \textcolor{blue}{For every task, we report the median performance across 5 runs. The tag ``1'' at the end of model setting indicates saving outliers. For second order momentum, we use transform=5 consistently. The statistics are obtained through the best results of each run, in fact there is no much difference gap between best results and final results except for MNLI task at 8F44 setting.}
    }
    \label{tab:glue-accuracy}
    \begin{tabular}{lccccccccc}
        \toprule
        Model         & MNLI & QNLI & QQP  & RTE  & SST-2 & MRPC & CoLA & STS-B & Avg.\\
        \midrule
        Ref.         & 90.2 & 94.7 & 92.2 & 86.6 &	96.4  & 90.9 & 68.0 & 92.4  & 88.9 \\
        \method(12/8/8/8)  & 90.5 & 94.6 & 91.9 & 84.8 & 96.4  & 90.7 & 67.1 & 92.3  & 88.5 \\
        \method(8/8/8/8)   & 90.4 & 94.6 & 91.9 & 85.6 & 96.4  & 90.0 & 64.6 & 92.1  & 88.2 \\
        \midrule
        FP32                   & 90.1 & 94.6 & 92.2 & 85.6 & 96.4 & 93.1 & 67.9 & 92.5 & - \\
        \method(8FFF-0)        & 89.8 & 94.5 & 91.9 & 86.3 & 96.3 & 92.9 & 68.8 & 92.2 & - \\
        \method(8FFF-1)        & 90.0 & 94.6 & 92.1 & 87.3 & 96.6 & 93.2 & 68.3 & 92.3 & - \\
        \method(FF4F-0)        & 90.1 & 94.6 & 92.2 & 82.7 & 96.6 & 92.4 & 67.5 & 92.3 & - \\
        \method(FF4F-1)        & 90.2 & 94.5 & 92.2 & 85.6 & 96.2 & 93.0 & 69.0 & 92.2 & - \\
        \method(FFF4)          & 90.4 & 94.9 & 92.2 & 86.3 & 96.4 & 93.2 & 66.6 & 92.4 & - \\
        \method(8F44-1)        & 89.8 & 94.5 & 92.0 & 85.9 & 96.2 & 93.2 & 67.3 & 92.2 & - \\
        \bottomrule
    \end{tabular}
\end{table}


\subsection{\textcolor{blue}{Experiment: Swin Transformer Classification}}

Table~\ref{tab:swin-quant-type-ablation} shows the effect of quantization methods on  accuracy for Swin-T ImageNet pretraining with AdamW. 
Like experiments in RoBERTa, we also compare with sublinear memory methods for second moment.

\begin{table}[htbp]
    \centering
    \caption{
    Left: Performance of Swin-T on ImageNet pretraining. \method(8F44) means that 8-bit parameter, 4-bit momentum, 4-bit second order momentum are used. The tag ``1'' at the end of model setting indicates saving outliers. For second order momentum, we use transform=5 consistently.
    Right: \textcolor{blue}{Effect of quantization methods on performance of Swin-T ImageNet pretraining with AdamW optimizer. We mainly focus on 4-bit momentum and 4-bit second moment, respectively. For second moment, we also compare with sublinear memory methods. 
    One run.}
    }
    \label{tab:swin-quant-type-ablation}
    \begin{tabular}{lc}
        \toprule
        Method         & top-1 acc. \\
        \midrule
        Ref.                   & 81.2 \\
        \midrule
        FP32                   & 81.1 \\
        \method(8FFF-0)        & 78.3 \\
        \method(8FFF-1)        & 80.2 \\
        \method(FF4F-0)        & unstable \\
        \method(FF4F-1)        & \textcolor{red}{76.98(stab.)} \\
        \method(FFF4)          & \textbf{81.2} \\
        \method(8FF4-1)        & 80.0/79.9(stab.) \\
        \method(8F44-1)        & \textcolor{red}{75.04(stab.)} \\
        \method(8444-1)        & 76.2 \\
        \bottomrule
    \end{tabular}
    \begin{tabular}{llc}
        \toprule
        Setting         & Method & top-1 acc. \\
        \midrule
        Ref.   & - & 81.2 \\
        FP32   & - & 81.1 \\
        8-bit Adam &  group & 81.2 \\
        \midrule
        4-bit Momentum & tensor & diverge \\
        4-bit Momentum & group  & $<$ 77.0 \\
        4-bit Momentum & dim0   & 79.0 \\
        % 4-bit Momentum & dim01  & 80.6 \\
        4-bit Momentum & rank-1 & 80.9 \\
        \midrule
        Sublinear & Adafactor & 80.7 \\
        Sublinear & SM3 & 80.7 \\
        4-bit Second moment & rank-1 & \textbf{81.1} \\
        \bottomrule
    \end{tabular}
\end{table}

\subsection{\textcolor{blue}{Experiment: Machine Translation}}

\begin{table}[htbp]
    \centering
    \caption{
    \textcolor{blue}{Effect of quantization methods on performance of Transformer on WMT14-en-de with Adam optimizer. We mainly focus on 4-bit momentum and 4-bit second moment, respectively. One run.}
    }
    \label{tab:mt-quant-type-ablation}
    \begin{tabular}{llc}
        \toprule
        Setting & Method         & SacreBLEU \\
        \midrule
        Ref.     & -              & ? \\
        FP32    & - & 26.8 \\
        \midrule
        4-bit Momentum & rank-1 & 26.8 \\
        4-bit Second moment & rank-1 & 26.7 \\
        \bottomrule
    \end{tabular}
\end{table}


% \subsection{\textcolor{blue}{Experiment: Diffusion Model}}

% \begin{table}[h]
%     \centering
%     \caption{
%     \textcolor{blue}{Effect of quantization methods on performance of Conditional VP ODE on CIFAR-10 pretraining with Adam optimizer. We mainly focus on 4-bit momentum and 4-bit second moment, respectively. For second moment, we also compare with sublinear memory methods.}
%     }
%     \label{tab:edm-fid}
%     \begin{tabular}{lc}
%         \toprule
%         Method         & FID \\
%         \midrule
%         Ref.                   & 1.79 \\
%         \midrule
%         FP32                   & 1.82 \\
%         % \method(8FFF-0)        & - \\
%         % \method(8FFF-1)        & - \\
%         \method(FF4F-0)        & - \\
%         % \method(FF4F-1)        & g43-ing \\
%         \method(FFF4)          & \textcolor{red}{74.33} \\
%         % \method(8FF4-1)        & - \\
%         \method(8F44-0)        & g43-done \\
%         % \method(8F44-1)        & lpmm8-done \\
%         \bottomrule
%     \end{tabular}
% \end{table}


\begin{table}[t]
    \centering
    \caption{Performance of ResNet-50 and Swin-T on ImageNet pretraining.
    \textcolor{blue}{
    The tag ``1'' at the end of model setting indicates saving outliers.
    For now, only 1 run in each setting is reported. deprecated}}
    \label{tab:abl-resnet-accuracy}
    \begin{tabular}{ccc}
        \toprule
        Model & Method & top-1 acc. \\
        % Model &  Method & Bits (param./grad./moment.) & Accuracy(\%) \\
        \midrule
        ResNet-18 & Ref. & 71.1 \\
        ResNet-50 & Ref. & 77.1 \\
        \midrule
        ResNet-18 & FP & 71.1 \\
        ResNet-50 & FP & 77.2 \\
        ResNet-18 & LPMM(12/8/8-0)  & 71.0 \\
        ResNet-50 & LPMM(12/8/8-0)  & 77.3 \\
        \midrule
        ResNet-50 & LPMM(8FF-0) & \textcolor{red}{75.7} \\
        ResNet-50 & LPMM(8FF-1) & \textcolor{red}{76.3} \\
        ResNet-50 & LPMM(FF4-0) & 76.6 \\
        ResNet-50 & LPMM(FF4-1) & \textbf{77.1} \\
        ResNet-50 & LPMM(8F4-0) & 75.0 \\
        ResNet-50 & LPMM(8F4-1) & 76.4 \\
        \bottomrule
    \end{tabular}
\end{table}

% \begin{table}[t]
%     \centering
%     \caption{Main results.} %The \method-SGDM with 12-bit parameters, 8-bit gradients, and 8-bit momentum match the performance of the full-precision baseline on the image classification task.\\}
%     \label{tab:main-results}
%     \begin{tabular}{lllccc}
%         \toprule
%         % Model & Method & top-1 acc. \\
%         % Model &  Method & Bits (param./grad./moment.) & Accuracy(\%) \\
%         Optimizer & Task & Model & Metric & Memory Saved & Time \\
%         \midrule
%         32-bit SGDM  & CLS & ResNet-50 & 77.2 & & \\
%         ~~4-bit LPMM & CLS & ResNet-50 & 76.8 & & \\
%         \midrule
%         32-bit AdamW & CLS & Swin-T & 81.2 & & \\
%         ~~4-bit LPMM & CLS & Swin-T & 81.2 & & \\
%         \midrule
%         32-bit AdamW     & GLUE & RoBERTa-Large & done & & \\
%         32-bit Adafactor & GLUE & RoBERTa-Large & done & & \\
%         ~~4-bit LPMM     & GLUE & RoBERTa-Large & ing & & \\
%         \midrule
%         32-bit AdamW     & MT & Transformer & TODO & & \\
%         32-bit Adafactor & MT & Transformer & TODO & & \\
%         ~~4-bit \method     & MT & Transformer & TODO & & \\
%         \midrule
%         32-bit AdamW     & MT & Transformer & TODO & & \\
%         32-bit Adafactor & MT & Transformer & TODO & & \\
%         ~~4-bit \method     & MT & Transformer & TODO & & \\
        
%         \bottomrule
%     \end{tabular}
% \end{table}


\begin{table}[h]
    \centering
    \caption{
    % Performance of RoBERTa-Large finetuning on GLUE and SQuAD with quantized optimizer states.
    % For every task, we report the median performance across 5 runs. 
    Some ablation results. 8-bit P gp=64, 4-bit M/S gp=rank-1 setting have 4 runs and 2 runs, respectively.
    \textcolor{blue}{
    % Effect of quantization methods on performance of RoBERTa-Large finetuning with Adam optimizer. We mainly focus on 4-bit momentum and 4-bit second moment, respectively. 
    % For second moment, we also compare with sublinear memory methods. 
    % For each run, we use the best result.
    % (1) we report rank-1 scaling, power-2 nearest for momentum and power-1 stochastic for square momentum. Use smaller group size such as 64 or 128 may produce better results. 
    % (2) Memory Saved todo.
    }
    }
    \label{tab:roberta-quant-type-ablation}
    \begin{tabular}{lcccccccc}
        \toprule
        Method   & MNLI & QNLI & QQP  & RTE  & SST-2 & MRPC & CoLA & STS-B \\
        \midrule
        Ref.    & 90.2 & 94.7 & 92.2 & 86.6 &	96.4 & 90.9 & 68.0 & 92.4  \\
        % FP32               & 90.1 & 94.6 & 92.2 & 85.6 & 96.4 & 93.1 & 67.9 & 92.5 \\
        FP32/32-bit AdamW & 90.2 & 94.9 & 92.2 & 85.2 & 96.3 & 93.2 & 66.9 & 92.3 \\
        % 4-bit LPMM  & 90.4 & 94.7 & 92.2 & 87.4 & 96.7 & 93.5 & 68.1 & 92.3 \\
        \midrule
        4-bit M group & 90.1 & 94.6 & 92.2 & 82.7 & 96.6 & 92.4 & 67.5 & 92.3 \\
        4-bit M rank-1  & 90.4 & 94.8 & 92.2 & 86.6 & 96.6 & 92.7 & 66.7 & 92.4 \\
        \midrule
        Adafactor & 90.6 & 94.7 & 91.7 & 84.8 & 96.2 & 92.3 & 67.8 & 92.3 \\
        \midrule
        8-bit P gp=64 & 90.0 & 94.5 & 92.1 & 87.0 & 96.4 & 93.4 & 68.9 & 92.3 \\
        4-bit M/S gp$\sim$rank-1 & 90.5 & 94.7 & 92.1 & 87.5 & 96.5 & 92.2 & 68.5 & 92.5 \\
        % 4-bit Momentum  & -     & 90.1 & 94.6 & 92.2 & 85.6 & 96.4 & 93.1 & 67.9 & 92.5 \\
        % \method(8FFF-0)        & 89.8 & 94.5 & 91.9 & 86.3 & 96.3 & 92.9 & 68.8 & 92.2 \\
        % \method(8FFF-1)        & 90.0 & 94.6 & 92.1 & 87.3 & 96.6 & 93.2 & 68.3 & 92.3 \\
        % \method(FF4F-0)        & 90.1 & 94.6 & 92.2 & 82.7 & 96.6 & 92.4 & 67.5 & 92.3 \\
        % \method(FF4F-1)        & 90.2 & 94.5 & 92.2 & 85.6 & 96.2 & 93.0 & 69.0 & 92.2 \\
        % \method(FFF4)          & 90.4 & 94.9 & 92.2 & 86.3 & 96.4 & 93.2 & 66.6 & 92.4 \\
        % \method(8F44-1)        & 89.8 & 94.5 & 92.0 & 85.9 & 96.2 & 93.2 & 67.3 & 92.2 \\
        \bottomrule
    \end{tabular}
\end{table}


==> src/a3-memory-saving.tex <==
\section{Memory Saving and Computational Overhead [TODO]}

In this section, we investigate memory saving and the overhead of \method. 
Tab.~\ref{tab:memory-saving} shows the memory saving and throughput on several benchmarks.
The model memory here is the peak memory, where all parameters, gradients and optimizer states stay in memory.
% and Tab.~\ref{tab:memory-saving-mb} shows the memory saving when microbatching is needed.
All measurements are performed under standard benchmarks, i.e. ImageNet classification for ResNet-50 and GLUE for RoBERTa-Large, and standard training configurations for all benchmarks.
Our \method-Adam saves up to 3.8 GB of GPU memory (about 72\%) for RoBERTa-Large and saves 62\% for ResNet-50,
which make the training(or finetuning) of large models more accessible.
% Runtime disscution
Besides, \method~would lead to a compuation overhead especially when the model is large, and the 8-bit Optimizer\citep{dettmers20218} has higher throughput than the baseline. 
This is due to \cite{dettmers20218} use operator fusion techniques to integrate the optimizer update, quantization into one single operator as a CUDA kernel, while \method~use CUDA only for quantization and PyTorch for other operations. 
This problem could be mitigated if the  \method~framwork is completely implemented in CUDA.
% This is due to the quantization operators that are complex and run multiple times of \method, 
% and is a trade-off with the amount of memory reduction.

In Tab.~\ref{tab:largest-trainable-model}, we investigate the largest trainable model in a single GPU with same memory under \method. We use a batch size of one and vary the depth and width respectively to explore the limit size. 
The GPU memory is consistently 11 GB for this comparison. 
Tab.~\ref{tab:memory-saving} and~\ref{tab:largest-trainable-model} both show \method~could attain a higher reduction rate for language tasks than vision tasks. This is because activation accounts more memory in vision tasks.

\begin{table}[h]
    \centering
    \caption{Saved Memory and Throughput on Various Tasks.} 
    \label{tab:memory-saving}
    \begin{tabular}{llllll}
        \toprule
        Method        & Model  & Model Mem & Saved Mem & Throughput(IPS) \\
        \midrule
        32-bit Momentum             &   ResNet-50       & 299.1 MB & 0.0 MB(0\%)    & 347.86  \\
        8-bit \citep{dettmers20218} &   ResNet-50       & 224.4 MB & 74.7 MB(25\%)  & 348.71  \\
        \method-Momentum(12/8/8)    &   ResNet-50       & 112.6 MB  & 186.5 MB(62\%) & 347.71  \\
        32-bit Adam                 &   RoBERTa-Large   & 5.3 GB & 0.0 GB(0\%)    & 186.2     \\
        8-bit \citep{dettmers20218} &   RoBERTa-Large   & 3.3 GB & 2.0 GB(38\%)   & 244.1     \\
        \method-Adam(12/8/8/8)      &   RoBERTa-Large   & 1.5 GB & 3.8 GB(72\%)   & 61.5      \\
        \bottomrule
    \end{tabular}
\end{table}

% \begin{table}[h]
%     \centering
%     \caption{Saved Memory and Throughput on Various Tasks.} 
%     \label{tab:memory-saving}
%     \begin{tabular}{llllll}
%         \toprule
%         Method        & Model  & Model Mem & Saved Mem & Throughput(IPS) \\
%         \midrule
%         32-bit Momentum             &   ResNet-50       & 197.2 MB & 0.0 MB(0\%)    & 347.86  \\
%         8-bit \citep{dettmers20218} &   ResNet-50       & 122.6 MB & 74.6 MB(38\%)  & 348.71  \\
%         \method-Momentum(12/8/8)    &   ResNet-50       & 79.5 MB  & 117.7 MB(60\%) & 347.71  \\
%         32-bit Adam                 &   RoBERTa-Large   & 4.0 GB & 0.0 GB(0\%)    & 186.2     \\
%         8-bit \citep{dettmers20218} &   RoBERTa-Large   & 2.0 GB & 2.0 GB(50\%)   & 244.1     \\
%         \method-Adam(12/8/8/8)      &   RoBERTa-Large   & 1.2 GB & 2.8 GB(70\%)   & 61.5      \\
%         \bottomrule
%     \end{tabular}
% \end{table}

% \begin{table}[h]
%     \centering
%     \caption{Saved Memory with Microbatching on Various Tasks.} 
%     \label{tab:memory-saving-mb}
%     \begin{tabular}{llll}
%         \toprule
%         Method        & Model & Model Mem w. MB & Saved Mem w. MB\\
%         \midrule
%         32-bit Momentum                     & ResNet-50 & 299.1 MB & 0.0 MB(0\%)    \\
%         8-bit \citep{dettmers20218}         & ResNet-50 & 224.4 MB & 74.7 MB(25\%)  \\
%         \method-Momentum(12/8/8)               & ResNet-50 & 112.6 MB & 186.5 MB(62\%) \\
%         32-bit Adam                         & RoBERTa-Large & 5.3 GB & 0.0 GB(0\%)    \\
%         8-bit \citep{dettmers20218}         & RoBERTa-Large & 3.3 GB & 2.0 GB(38\%)  \\
%         \method-Adam(12/8/8/8)                 & RoBERTa-Large & 1.5 GB & 3.8 GB(72\%) \\
%         \bottomrule
%     \end{tabular}
% \end{table}

\begin{table}[h]
    \centering
    \caption{Largest trainable(or finetunable) Model with same GPU memory.}
    \label{tab:largest-trainable-model}
    \begin{tabular}{cc|ccc}
        \toprule
        % Model &  Method & Bits (param./grad./moment.) & Accuracy(\%) \\
                 & \multirow{2}{*}{Dim} & \multicolumn{3}{c}{Maximum Value}    \\
                 &                       & FP & \citep{dettmers20218} & \method \\
        \midrule
        \multirow{2}{*}{ResNet-152}     & D     & 712   & 804   & 1016                  \\
                                        & W     & 296   & 340   & 472                   \\
        \multirow{2}{*}{RoBERTa-Large}  & D     & 40    & 72    & 148                   \\
                                        & W     & 1312  & 2048  & 3232                  \\
        \bottomrule
    \end{tabular}
\end{table}




==> src/a4-addi-related-work.tex <==
\newpage
\section{Detailed Comparison of \method~with Low-bit Training and Quantized Training [ongoing]}

To clarify the difference in contributions and techniques between \method~and other work, including quantized training, communication efficient training, memory efficient training, etc., we summarize the computation bits and storage bits of existing works. 
First, we would like to point out that there are two types of numerical precision in a low-precision training system:
\begin{itemize}
    \item \emph{Storage bitwidth} characterizes the numerical precision of parameters, gradients, and momentums stored in the memory, where we use 
    \begin{itemize}
        \item parameter storage bitwidth (PSB) to refer
    the bitwidth of the stored parameters (a.k.a., primal/master parameters or latent weights);
    \item gradient storage bitwidth (GSB) to refer the bitwidth of stored (parameter) gradients, which are fed into the optimizer;
    \item momentum storage bit (MSB) to refer the bitwidth of stored momentums.
    \end{itemize}
    \item \emph{Computation bitwidth} characterizes the numerical precision of the computing kernels (GEMM, conv, etc.), where we use
    \begin{itemize}
        \item parameter computation bitwidth (PCB) to refer the bitwidth of parameter inputs to forward operators;
        \item gradient computation bitwidth (GCB) to refer the bitwidth of (activation) gradient inputs to backward operators;
        \item momentum computation bitwidth (MCB) to refer the bitwidth of momentum in optimizer operators.
    \end{itemize}
\end{itemize}

We list the computation and storage bits of existing works Tab.~\ref{tab:clarification-of-lpmm}. 
Existing low-precision training methods (DoReFa, WAGE, FP8, INT8, GradScale) mainly consider reducing the computation bitwidth. The parameters are stored in high-precision (16 or 32) and then converted to low-precision (4 or 8) for computing forward and backward propagation. Among these methods, LPMM can achieve lowest storage bits. Meanwhile, those memory efficient quantized training methods (WAGEUBN, FXPNet) suffer from major accuracy loss, as shown in Tab.~\ref{tab:experiment-comparison}.


%Many work use multiple bit-width setting for studying the sensitivity, 
%and here we list the principally claimed setting in their work. 

\begin{table}[h]
    \centering
    \caption{Difference between \method~and other low-bit training works. p. stands for parameter, m. stands for moment or optimizer states. ``-'' stands for not considered or mentioned.
    %Here we do not consider the specialized techniques for specific parameters such as BN, last layer, etc.
    % , which probably indicates 32-bit (sometimes 16-bit) is adopted. 
    } 
    \label{tab:clarification-of-lpmm}
    \begin{tabular}{cl|cccccc}
        \toprule
            &       & \multicolumn{3}{c}{Computation Bits}    & \multicolumn{3}{c}{Storage Bits}  \\
        Type &  Method                      & p.    & g.    & m.    & p.    & g.    & m.        \\
        \midrule
        &DoReFa-Net\citep{zhou2016dorefa}   & 1     & 6     & -     & 32    & 32    & -         \\
        &WAGE\citep{wang2018training}        & 8     & 8/16  & 13    & 24    & \textbf{8}     & 15        \\
        &WAGEUBN\citep{yang2020training}    & 8     & 8/16  & 13    & 24    & \textbf{8}     & 15        \\
Quantized&FP8 training\citep{wang2018training}& 8   & 8     & 16    & 16    & 16    & 16        \\
Training&INT8\citep{zhu2020towards}         & 8     & 8     & -     & 32    & 32    & -         \\
        &FXPNet\citep{chen2017fxpnet}       & 1     & 12    & 32    & \textbf{12}    & 12    & 12        \\
        &GradScale\citep{sun2020ultra}      & 4     & 4     & -     & 16/32 & 16    & -         \\
        \midrule
        &LP-SGD\citep{li2017training}       & 32    & 32    & -     & \textbf{1}     & 32    & -         \\
        &HALP\citep{de2018high}             & 32    & 32    & -     & 32    & 32    & -         \\
        &SWALP\citep{yang2019swalp}        & 32    & 32    & 32    & \textbf{9}/32  & \textbf{8}     & \textbf{8}         \\
% Training&8-bit Optim.\citep{dettmers20218}  & 32    & 32    & 32    & 32    & 32    & \textbf{8}         \\
% &\method(ours)                      & 32    & 32    & 32    & \textbf{12}    & \textbf{8}     & \textbf{8}\\
        \bottomrule
    \end{tabular}
\end{table}


% \begin{table}[t]
% \caption{Comparison of validation accuracy for ResNet 18/50 on ImageNet}
%     \label{tab:appendix-accuracy}
%     \centering
%     \begin{tabular}{c|ccccc}
%             \toprule
%         Method & p. & g. & m. & acc. (R18) & acc. (R50) \\
%         \midrule
%         WAGEUBN &  &  & & & \\ 
%         FP8 &  &  & & & \\ 
%         FXPNet &  &  & & & \\ 
%         GradScale &  &  & & & \\ 
%         LPMM (ours) &  &  & & & \\ 
%          \bottomrule
%     \end{tabular}
% \end{table}

% Additionally, we give some remarks about the Tab.~\ref{tab:clarification-of-lpmm}. 
% Note that some data in the table are inferred by our understanding about the original papers since the bit-widths of these data are not given exactly. These include the MSB of WAGEUBN, the PSB and GSB of GradScale.
% Secondly, while some work have low GSB, they did not talk about the persistent storage about gradients 
% (e.g. how to gradient accumulation), including DoReFa-Net and WAGEUBN. Since they have inconsistent PSB and GSB, the simple gradient accumulation operation is not obvious.
Next, we compare LPMM with existing methods in more detail at the aspects of contributions, experiments and how stochastic rounding is used.

% Remark
% \begin{enumerate}
%     \item Report the main claimed bit-width.
%     \item About the grad storage bit.
%     \item momentum computation and storage bit of WAGEUBN
%     \item p. and g. storage bit of GradScale
% \end{enumerate}

% \bingrui{Explanation about the Grad. storage bit.}
% no discussion about how to persistent store the gradients (i.e. no way for gradient accumulation)
% - DoReFa-Net, WAGEUBN, 
\paragraph{Difference on Contributions}
First, we talk about the quantized training.
DoReFa-Net, INT8 and GradScale mainly focus on the acceleration of the training process.
While they also can reduce the training memory footprint via low-bit kernel, the reduction is nearly independent to the model size. 
On the other hand, FP8 training, WAGEUBN and FXPNet focus on both training acceleration and memory footprint reduction (of the model storage).
For communication efficient training, they quantize the gradient into lower bits for more efficient communication in distributed scenario.
While the goals are different, both communication efficient training and \method~use a lower GSB,
which is necessary and beneficial to persistent storage of gradients.

For memory efficient training, we mainly refer to the work focusing on the quantization on post-update parameters and other values.
LP-SGD only stays in theoretical analysis.
HALP quantized the post-update parameters though, they store the main parameters in full-precision and in fact are intended to use low-precision computations.
SWALP extended the HALP but in fact stored high-precision parameters as well.
Unlike others, 8-bit Optimizer focused on reducing the storage of optimizer states instead of primal parameters, 
in fact the two are proportional (even equal).
Actually, WAGEUBN, FXPNet and SWALP did not report the memory saving which probably indicates they only conducted simulation experiments, and to our best knowlegde, we are the first to store low-bit parameters with $<$16-bit in realistic scenarios.
% \bingrui{TODO: which really reduce memory on GPU?}
% \bingrui{Explanation about the contributions/goals}
% \begin{enumerate}
%     \item DoReFa-Net\citep{zhou2016dorefa}: completely focused on 
%     \item FP8 training: both acceleration and memory saving
%     \item WAGEUBN: both acceleration and memory saving
%     \item INT8: only acceleration
%     \item FXPNet: both acceleration and memory saving
%     \item GradScale: only acceleration
% \end{enumerate}

\paragraph{Difference on Experimental Results}
Here we mainly talk about the experiments related to low-precision model memory.
As shown in Tab.~\ref{tab:experiment-comparison},
the performance of WAGEUBN and SWALP are lossy compared with full-precision baseline on ImageNet dataset, while FP8 training and GradScale are nearly lossless on both CIFAR and ImageNet under their mainly claimed setting. The FXPNet has lossless accuracy on CIFAR but no experiments on ImageNet.
Actually, there is an intrinsic complexity gap between the two datasets. 
From our observation, 8-bit primal parameters are enough for CIFAR10 to attain lossless accuracy, but 12-bit parameters are needed for ImageNet. 

In other words, to our best knowledge, there are no comparable performance with full-precision baseline under the primal parameters less than 16-bit in previous work. However, \method~attain lossless accuracy using 12-bit parameter.
For other values, QSGD and 8-bit Optimizer can achieve lossless performance compared with full-precision using 4/8-bit gradient and 8-bit optimizer states, respectively.

\begin{table}[h]
    \centering
    \caption{Comparison of experiments between \method~and comparable previous work for ResNet on ImageNet
    } 
    \label{tab:experiment-comparison}
    \begin{tabular}{l|llllll}
        \toprule
                                            &           &       \multicolumn{3}{c}{Storage Bits}        & \\
        Method                              & Model     & p.    & g.    & m.    & Acc.      & FP Baseline\\
        \midrule
        WAGEUBN\citep{yang2020training}     & ResNet-18 & 24    & 8     & 15    & 67.40     & 68.70     \\
        FP8 training\citep{wang2018training}& ResNet-18 & 16    & 16    & 16    & 66.95     & 67.43     \\
        FXPNet\citep{chen2017fxpnet}        & -         & 12    & 12    & 12    & -         & -         \\
        GradScale\citep{sun2020ultra}       & ResNet-18 & 16/32 & 16    & -     & 68.27     & 69.40     \\
        SWALP\citep{yang2019swalp}          & ResNet-18 & 9/32  & 32    & 32    & 65.11     & 69.51     \\
        \method(ours)                       & ResNet-18 & 12    & 8     & 8     & 71.0      & 71.1      \\
        \method(ours)                       & ResNet-18 & 8     & 8     & 8     & 69.2      & 71.1      \\
        \midrule
        QSGD\citep{alistarh2017qsgd}        & ResNet-50 & 32    & 4/8   & 8     & 74.76     & 74.68     \\
        8-bit Optim.\citep{dettmers20218}   & ResNet-50 & 32    & 32    & 8     & 77.2      & 77.1      \\
        \method(ours)                       & ResNet-50 & 12    & 8     & 8     & 77.3      & 77.2      \\
        \bottomrule
    \end{tabular}
\end{table}


% Since the full-precision baseline has different accuracy, 
% we do not compare the accuracy with these work. 

% \bingrui{Explanation about the experiments}
% \begin{enumerate}
%     \item DoReFa-Net: lossy in imagenet
%     \item FP8 training: nearly lossless in cifar and imagenet
%     \item WAGEUBN: lossy in imagenet
%     \item INT8: nearly lossless in cifar and imagenet
%     \item FXPNet: no results on imagenet
%     \item GradScale: nearly lossless in cifar and imagenet
% \end{enumerate}
\paragraph{How SR is used}
Then, we discuss about how stochastic rounding~\citep{gupta2015deep} is used in various work.
Firstly, FXPNet and GradScale did not use stochastic rounding technique in their main contribution.
DoReFa-Net, WAGEUBN, INT8 only use stochastic rounding in the quantizer before forward and backward operations to 
generate a low-bit input to the low-bit kernel, 
which is completely different from our setting.
The FP8 training, HALP, SWALP uses stochastic rounding in parameter update, same as \method.
However, we dive deeply into why stochastic rounding is necessary from network training dynamics and parameter distribution,
while they either give accuracy gap with or without stochastic rounding, or not concern about the SR technique itself.
Lastly, 8-bit Optimizer and signSGD did not use stochastic rounding, 
and QSGD used stochastic rounding on gradients, which we think possibly make a different roles from that on parameters since the difference on distributions. Again, QSGD also did not concern about the why SR is necessary.
In short, we empirically analyze that why the unbiasedness of SR is necessary from the training dynamics and parameter distribution, which is not given in previous work.

% \bingrui{Explanation about how does the stochastic rounding is used?}
% \begin{enumerate}
%     \item DoReFa-Net: used in forward and backward operations
%     \item FP8 training: used in weight update(as ours), but we dive deeply into why SR is needed in network training dynamics.
%     \item WAGEUBN: used for only gradient in backward operations
%     \item INT8: used in forward and backward operations
%     \item FXPNet: stochastic rounding is not used
%     \item GradScale: stochastic rounding is not used
% \end{enumerate}


==> src/a5-log-quantization.tex <==
\section{\textcolor{blue}{Quantization Guided by Near-Log-Normality}}

\cite{chmiel2021neural} oberserve that the neural gradients(gradients w.r.t. intermediate neural layer outputs) are near-log-normal distributed, inspiring us that the empirical distribution of optimizer states would be near-log-normal as well. Under this assumption, we can use the well-established methods for quantizing the normal distribution~\citep{lin2016fixed}. 
For completeness, here we state how to quantize the normal distribution in \cite{lin2016fixed}. 
\begin{enumerate}
    \item Calculate the effective standard deviation $\zeta$. For an ideal Gaussian, $\zeta = \sigma$ exactly. If the empirical distribution has longer tails than Gaussian, we usually set $\zeta > \sigma$.
    \item Calculate the effective stepsize via $\delta = \sigma * \textit{Stepsize}(b)$, where the \textit{Stepsize} function is given by \cite{shi1999image}, which is the optimal symmetric uniform quantizer i.e. the stepsize, for Gaussian distribution with fixed bit-width in the sense of minimizing the SQNR.
    \item The zero can be included or excluded according to the situation. Then all the quantization points can be determined according to stepsize and number of points.
\end{enumerate}
Below, we call this method normal method or log-normal method.

Therefore, we only need to verify the log-normal distribution assumption. Fig.~\ref{TODO} shows the histogram of optimizer states of one tensor in Swin-T. The distribution is close to a normal shape except that it is asymmetric. The characteristic of asymmetry brings more difficulties in quantization. 

\textcolor{blue}{Currently, we experimentally get both better SQNR and relative error on real log-normal data via log-noraml method.
But for optimizer states checkpoint, the log-normal method perform worse than rank-1, dim0 (scale-based) method due to the asymmetry.
One of the possible solution is to translate left the quantization points. The problem lies in how far should we move.
Second possible solution is to apply an invertible transform, such as power transform, to reduce the skewness of the distribution. Not exploring enough.
}


==> src/a7-quantization-error-analysis.tex <==
\newpage
\section{Quantization Error Analysis}

\bingrui{0515: what to write in this section}
% \textcolor{blue}{Some remarks, do not display: Note that better relative error may not imply better performance. }
% \begin{itemize}
%     \item On Transformer Adam setting
%     \item Straightforward relative error, scalar on a tensor
%     \item histogram and quantization error per bin, curve on a tensor, qualitively
%     \item Note that for linear quantization, absolute error for each bin may be similar and even identical.
% \end{itemize}

Since stochastic rounding is always worse than nearest rounding in the sense of quantization error. In this section, we use nearest rounding consistently. 

\subsection{Quantization Error on First Moment}

\begin{table}[htbp]
    \centering
    \caption{Relative quantization error for the first moment in AdamW optimizer states via different
quantization methods. Nearest Rounding is used. 
Results show averaged error across all tensors in Swin-T model.}
    \label{tab:approximation-err-fm-swin-avg-all}
    \begin{tabular}{lcccccc}
        \toprule
        Quant. Map & rank1-group & group128 & group2048 & rank1 & dim0 & dim1 \\
        \midrule
DE & 14.9\% & 16.7\% & 21.4\% & 15.8\% & 18.9\% & 18.2\% \\
FP & 12.5\% & 16.0\% & 25.8\% & 13.5\% & 20.1\% & 17.2\% \\
P1 & 11.8\% & 16.6\% & 31.9\% & 12.9\% & 21.9\% & 18.6\% \\
P2 & \textbf{11.2\%} & 12.6\% & 17.1\% & 11.8\% & 14.6\% & 13.8\% \\
    \bottomrule
    \end{tabular}
\end{table}

\begin{table}[htbp]
    \centering
    \caption{Relative quantization error for the first moment in AdamW optimizer states via different
quantization methods. Nearest Rounding is used. 
Results show maximal error across all tensors in Swin-T model.}
    \label{tab:approximation-err-fm-swin-max-all}
    \begin{tabular}{lcccccc}
        \toprule
        Quant. Map & rank1-group & group128 & group2048 & rank1 & dim0 & dim1 \\
        \midrule
DE & 15.9\% & 18.2\% & 23.8\% & 19.5\% & 24.4\% & 22.3\% \\
FP & 14.7\% & 21.8\% & 37.4\% & 20.5\% & 38.3\% & 28.0\% \\
P1 & 16.4\% & 30.3\% & 67.8\% & 21.4\% & 59.8\% & 37.9\% \\
P2 & \textbf{12.0\%} & 13.9\% & 21.2\% & 14.7\% & 22.1\% & 17.9\% \\
    \bottomrule
    \end{tabular}
\end{table}


\begin{table}[htbp]
    \centering
    \caption{Relative approximation error for the first moment in AdamW optimizer states via different
quantization methods. Nearest Rounding is used. 
Results show mean $\pm$ standard deviation of the attention projection layer ($\Wv^Q$, $\Wv^K$ and $\Wv^V$) accorss all transformers block in Swin-T model.}
    \label{tab:approximation-err-ablation-swin-wqkv}
    \begin{tabular}{lcccccc}
        \toprule
                  & group128 & group2048 & rank-1 & dim0 & dim1 \\
        \midrule
dynamic exponent & 0.24 $\pm$ 0.04 & 0.28 $\pm$ 0.05 & 0.23 $\pm$ 0.02 & 0.25 $\pm$ 0.03 & 0.29 $\pm$ 0.04 \\
floating point & 0.31 $\pm$ 0.07 & 0.43 $\pm$ 0.07 & 0.31 $\pm$ 0.06 & 0.35 $\pm$ 0.07 & 0.45 $\pm$ 0.04 \\
power-1 & 169 $\pm$ 544 & 405 $\pm$ 1e3 & 9.69 $\pm$ 11.6 & 128 $\pm$ 398 & 19.6 $\pm$ 1.95 \\
power-2 & 11.4 $\pm$ 36.2 & 27.1 $\pm$ 88.5 & 0.79 $\pm$ 0.77 & 8.71 $\pm$ 26.5 & 1.44 $\pm$ 1.28 \\
        \bottomrule
    \end{tabular}
\end{table}

\begin{table}[htbp]
    \centering
    \caption{Relative approximation error for the first moment in AdamW optimizer states via different
quantization methods. Nearest Rounding is used. 
Results show mean $\pm$ standard deviation of the attention output layer ($\Wv^O$) accorss all transformers block in Swin-T model.}
    \label{tab:approximation-err-ablation-swin-wo}
    \begin{tabular}{lcccccc}
        \toprule
                  & group128 & group2048 & rank-1 & dim0 & dim1 \\
        \midrule
dynamic exponent & 0.22 $\pm$ 0.02 & 0.26 $\pm$ 0.03 & 0.21 $\pm$ 0.00 & 0.23 $\pm$ 0.01 & 0.22 $\pm$ 0.01 \\
floating point & 0.28 $\pm$ 0.06 & 0.36 $\pm$ 0.07 & 0.25 $\pm$ 0.01 & 0.30 $\pm$ 0.05 & 0.28 $\pm$ 0.02 \\
power-1 & 2.44 $\pm$ 1.27 & 4.19 $\pm$ 2.78 & 1.91 $\pm$ 0.34 & 2.60 $\pm$ 0.84 & 2.26 $\pm$ 0.57 \\
power-2 & 0.30 $\pm$ 0.09 & 0.43 $\pm$ 0.18 & 0.26 $\pm$ 0.02 & 0.32 $\pm$ 0.06 & 0.29 $\pm$ 0.04 \\
        \bottomrule
    \end{tabular}
\end{table}

\begin{table}[htbp]
    \centering
    \caption{Relative approximation error for the first moment in AdamW optimizer states via different
quantization methods. Nearest Rounding is used. 
Results show mean $\pm$ standard deviation of the MLP projection layer ($\Wv^1$) accorss all transformers block in Swin-T model.}
    \label{tab:approximation-err-ablation-swin-w1}
    \begin{tabular}{lcccccc}
        \toprule
                  & group128 & group2048 & rank-1 & dim0 & dim1 \\
        \midrule
        dynamic exponent & 0.25 $\pm$ 0.03 & 0.31 $\pm$ 0.04 & 0.24 $\pm$ 0.02 & 0.26 $\pm$ 0.02 & 0.25 $\pm$ 0.02 \\ 
        floating point & 0.36 $\pm$ 0.05 & 0.51 $\pm$ 0.05 & 0.32 $\pm$ 0.04 & 0.40 $\pm$ 0.06 & 0.36 $\pm$ 0.05 \\
        power-1 &  14.1 $\pm$ 27.0 & 39.9 $\pm$ 79.1 & 4.25 $\pm$ 2.23 & 10.6 $\pm$ 10.3 & 5.52 $\pm$ 2.77 \\
        power-2 &  1.09 $\pm$ 1.78 & 2.80 $\pm$ 5.21 & 0.43 $\pm$ 0.15 & 0.86 $\pm$ 0.69 & 0.52 $\pm$ 0.18 \\
        \bottomrule
    \end{tabular}
\end{table}

\begin{table}[htbp]
    \centering
    \caption{Relative approximation error for the first moment in AdamW optimizer states via different
quantization methods. Nearest Rounding is used. 
Results show mean $\pm$ standard deviation of the MLP output layer ($\Wv^2$) accorss all transformers block in Swin-T model.}
    \label{tab:approximation-err-ablation-swin-w2}
    \begin{tabular}{lcccccc}
        \toprule
                  & group128 & group2048 & rank-1 & dim0 & dim1 \\
        \midrule
dynamic exponent & 0.23 $\pm$ 0.02 & 0.27 $\pm$ 0.03 & 0.22 $\pm$ 0.01 & 0.26 $\pm$ 0.03 & 0.22 $\pm$ 0.01 \\
floating point & 0.29 $\pm$ 0.06 & 0.40 $\pm$ 0.07 & 0.27 $\pm$ 0.03 & 0.38 $\pm$ 0.08 & 0.28 $\pm$ 0.03 \\
power-1 & 5.18 $\pm$ 6.99 & 10.4 $\pm$ 14.4 & 5.06 $\pm$ 9.78 & 11.0 $\pm$ 20.0 & 5.21 $\pm$ 9.81 \\
power-2 & 0.48 $\pm$ 0.46 & 0.84 $\pm$ 0.94 & 0.48 $\pm$ 0.66 & 0.88 $\pm$ 1.33 & 0.49 $\pm$ 0.66 \\
        \bottomrule
    \end{tabular}
\end{table}


\begin{table}[htbp]
    \centering
    \caption{Relative approximation error for the first moment in AdamW optimizer states via different
quantization methods. Nearest Rounding is used. 
Results show mean $\pm$ standard deviation of the attention projection layer ($\Wv^Q$, $\Wv^K$ and $\Wv^V$) accorss all transformers block in GPT-2 medium model.}
    \label{tab:approximation-err-ablation-gpt2-wqkv}
    \begin{tabular}{lcccccc}
        \toprule
                  & group128 & group2048 & rank-1 & dim0 & dim1 \\
        \midrule
dynamic exponent & 0.23 $\pm$ 0.01 & 0.29 $\pm$ 0.01 & 0.27 $\pm$ 0.02 & 0.31 $\pm$ 0.04 & 0.30 $\pm$ 0.03 \\
floating point & 0.29 $\pm$ 0.01 & 0.46 $\pm$ 0.04 & 0.40 $\pm$ 0.03 & 0.49 $\pm$ 0.05 & 0.46 $\pm$ 0.04 \\
power-1 & 8.11 $\pm$ 19.0 & 24.2 $\pm$ 53.0 & 19.8 $\pm$ 56.7 & 28.0 $\pm$ 57.7 & 37.5 $\pm$ 102 \\
power-2 & 0.68 $\pm$ 1.27 & 1.76 $\pm$ 3.53 & 1.48 $\pm$ 3.78 & 2.00 $\pm$ 3.84 & 2.64 $\pm$ 6.79 \\
        \bottomrule
    \end{tabular}
\end{table}

\begin{table}[htbp]
    \centering
    \caption{Relative approximation error for the first moment in AdamW optimizer states via different
quantization methods. Nearest Rounding is used. 
Results show mean $\pm$ standard deviation of the attention output layer ($\Wv^O$) accorss all transformers block in GPT-2 medium model.}
    \label{tab:approximation-err-ablation-gpt2-wo}
    \begin{tabular}{lcccccc}
        \toprule
                  & group128 & group2048 & rank-1 & dim0 & dim1 \\
        \midrule
dynamic exponent & 0.20 $\pm$ 0.00 & 0.24 $\pm$ 0.01 & 0.22 $\pm$ 0.00 & 0.23 $\pm$ 0.01 & 0.27 $\pm$ 0.02 \\
floating point & 0.24 $\pm$ 0.00 & 0.33 $\pm$ 0.02 & 0.27 $\pm$ 0.01 & 0.29 $\pm$ 0.02 & 0.40 $\pm$ 0.04 \\
power-1 & 2.50 $\pm$ 0.90 & 4.46 $\pm$ 1.92 & 3.14 $\pm$ 1.22 & 3.44 $\pm$ 1.32 & 7.32 $\pm$ 3.27 \\
power-2 & 0.30 $\pm$ 0.06 & 0.45 $\pm$ 0.13 & 0.35 $\pm$ 0.08 & 0.38 $\pm$ 0.09 & 0.64 $\pm$ 0.22 \\
        \bottomrule
    \end{tabular}
\end{table}

\begin{table}[htbp]
    \centering
    \caption{Relative approximation error for the first moment in AdamW optimizer states via different
quantization methods. Nearest Rounding is used. 
Results show mean $\pm$ standard deviation of the MLP projection layer ($\Wv^1$) accorss all transformers block in GPT-2 medium model.}
    \label{tab:approximation-err-ablation-gpt2-w1}
    \begin{tabular}{lcccccc}
        \toprule
                  & group128 & group2048 & rank-1 & dim0 & dim1 \\
        \midrule
dynamic exponent & 0.25 $\pm$ 0.01 & 0.30 $\pm$ 0.03 & 0.25 $\pm$ 0.02 & 0.31 $\pm$ 0.03 & 0.26 $\pm$ 0.03 \\
floating point & 0.36 $\pm$ 0.02 & 0.47 $\pm$ 0.04 & 0.36 $\pm$ 0.05 & 0.49 $\pm$ 0.04 & 0.39 $\pm$ 0.07 \\
power-1 & 7.45 $\pm$ 5.64 & 14.9 $\pm$ 11.2 & 6.80 $\pm$ 4.78 & 16.9 $\pm$ 12.1 & 9.04 $\pm$ 6.44 \\
power-2 & 0.65 $\pm$ 0.37 & 1.14 $\pm$ 0.73 & 0.61 $\pm$ 0.32 & 1.28 $\pm$ 0.79 & 0.76 $\pm$ 0.43 \\
        \bottomrule
    \end{tabular}
\end{table}

\begin{table}[htbp]
    \centering
    \caption{Relative approximation error for the first moment in AdamW optimizer states via different
quantization methods. Nearest Rounding is used. 
Results show mean $\pm$ standard deviation of the MLP output layer ($\Wv^2$) accorss all transformers block in GPT-2 medium model.}
    \label{tab:approximation-err-ablation-gpt2-w2}
    \begin{tabular}{lcccccc}
        \toprule
                  & group128 & group2048 & rank-1 & dim0 & dim1 \\
        \midrule
dynamic exponent & 0.21 $\pm$ 0.00 & 0.25 $\pm$ 0.01 & 0.23 $\pm$ 0.01 & 0.23 $\pm$ 0.01 & 0.31 $\pm$ 0.04 \\
floating point & 0.24 $\pm$ 0.01 & 0.35 $\pm$ 0.03 & 0.29 $\pm$ 0.02 & 0.29 $\pm$ 0.02 & 0.49 $\pm$ 0.05 \\
power-1 & 2.67 $\pm$ 0.56 & 5.98 $\pm$ 1.88 & 3.67 $\pm$ 0.88 & 3.77 $\pm$ 0.90 & 16.8 $\pm$ 13.7 \\
power-2 & 0.31 $\pm$ 0.04 & 0.55 $\pm$ 0.12 & 0.39 $\pm$ 0.06 & 0.40 $\pm$ 0.06 & 1.27 $\pm$ 0.87 \\
        \bottomrule
    \end{tabular}
\end{table}

\subsection{Quantization Error on Second Moment}

\bingrui{The difficulty of pretrained task over finetuning task, by maximal relative quantization error on second moment for swin-T and LM.}

\begin{table}[htbp]
    \centering
    \caption{Relative quantization error for the second moment in AdamW optimizer states via different
quantization methods. Nearest Rounding is used. 
Results show averaged error across all tensors in Swin-T model.}
    \label{tab:approximation-err-sm-swin-avg-all}
    \begin{tabular}{lcccccc}
        \toprule
        Quant. Map & rank1-group & group128 & group2048 & rank1 & dim0 & dim1 \\
        \midrule
DE & 6.3e+04\% & 1.4e+05\% & 4.9e+05\% & 1.5e+02\% & 3.4e+04\% & 3.3e+05\% \\
DE w/o. zero & 14.2\% & 26.5\% & 31.6\% & 11.0\% & 26.7\% & 14.6\% \\
P1 & 19.9\% & 36.0\% & 49.8\% & 17.6\% & 38.9\% & 27.3\% \\
P2 & 13.1\% & 26.2\% & 33.3\% & 10.0\% & 26.8\% & 14.7\% \\
    \bottomrule
    \end{tabular}
\end{table}

% \begin{table}[htbp]
%     \centering
%     \caption{Relative quantization error for the second moment in AdamW optimizer states via different
% quantization methods. Nearest Rounding is used. 
% Results show maximal error across all tensors in Swin-T model.}
%     \label{tab:approximation-err-sm-swin-max-all}
%     \begin{tabular}{lcccccc}
%         \toprule
%         Quant. Map & rank1-group & group128 & group2048 & rank1 & dim0 & dim1 \\
%         \midrule
% DE & 15.9\% & 18.2\% & 23.8\% & 19.5\% & 24.4\% & 22.3\% \\
% FP & 14.7\% & 21.8\% & 37.4\% & 20.5\% & 38.3\% & 28.0\% \\
% P1 & 16.4\% & 30.3\% & 67.8\% & 21.4\% & 59.8\% & 37.9\% \\
% P2 & \textbf{12.0\%} & 13.9\% & 21.2\% & 14.7\% & 22.1\% & 17.9\% \\
%     \bottomrule
%     \end{tabular}
% \end{table}


==> src/previouts.tex <==
\section{Previous Scripts}

\subsection{Quantized Optimizer with Momentum}
\textbf{Basic GD (1x space)}
\begin{align*}
\theta_{t+1}\leftarrow Q(\theta_t - \eta \nabla f(\theta_t))
\end{align*}

Discretization error is $O(\theta/B)$, when $\eta \nabla f \ll \theta/B$, the algorithm stucks.

\textbf{Batching (3x space)}
\begin{align*}
\theta_{t+1}&\leftarrow Q(\theta_t - \eta g_{t, N})\\
g_{t, 0}&\leftarrow 0 \\
g_{t, i+1}&\leftarrow Q(g_{t, i} + \nabla f(\theta_{t} - \eta g_{t, i}))
\end{align*}
The magnitude of $g_{t, N}$ is $O(N \nabla f)$, its discretization error is $O(N\nabla f / B)$. Now, the algorithm only stucks when $N\eta\nabla f \ll \theta/B$, which is $N$ times better than the basic algorithm. Meanwhile, $g$ plays a role like momentum. 

\paragraph{Remark: }
Why batching helps? It is essentially enlarging the learning rate... When $\eta$ is large, we have 
\begin{align*}
\E{\norm{\epsilon_t}^2}\le \eta^2 \norm{\nabla f(\hat\theta_t)}^2 + PD.
\end{align*}
In this case, we have 
\begin{align*}
\E{f(\hat\theta_{t+1})}\le f(\hat\theta_t) - \eta(1-\tfrac{L\eta}{2}) \norm{\nabla f(\hat\theta_t)}^2 + \tfrac{LPD}{2}.
\end{align*}
When $\eta \le \frac{1}{L}$, 
organizing the terms yields
\begin{align*}
\E{\frac{1}{T}\sum_{t=1}^{T}\norm{\nabla f(\hat\theta_t)}^2}
\le \frac{2(f(\hat\theta_1)-f_*)}{T\eta} + \frac{LPD}{\eta}.
\end{align*}

\paragraph{Microbatching (2x space)}
\begin{align*}
\theta_{t+1}&\leftarrow Q(\theta_t - \eta g_{t, N})\\
g_{t, 0}&\leftarrow 0 \\
g_{t, i+1}&\leftarrow Q(g_{t, i} + \nabla f(\theta_{t}))
\end{align*}
This is equivalent with an SGD with a large batch size of $N$.

\paragraph{Momentum (2x space)}7
\begin{align*}
v_{t+1}&\leftarrow Q(\beta v_t + (1-\beta)\nabla f(\theta_t))\\
\theta_{t+1}&\leftarrow Q(\theta_T - \eta v_{t+1})
\end{align*}
Is this is ideal way to parameterize it? The following might be better?
\begin{align*}
v_{t+1}&\leftarrow Q(v_t + (1-\beta)/\beta\nabla f(\theta_t))\\
\theta_{t+1}&\leftarrow Q(\theta_T - \eta \beta^t v_{t+1})
\end{align*}

\paragraph{Momentum with Microbatching (2x space)}
\begin{align*}
v_{t+1, 0}&\leftarrow Q(\beta v_{t, N})\\
v_{t+1, i+1}&\leftarrow Q(v_{t+1, i} + (1-\beta) \nabla f_i(\theta_t))\\
\theta_{t+1}&\leftarrow Q(\theta_T - \eta v_{t+1, N})
\end{align*}
This is equivalent with MomentumSGD with a batch size of $N$.

\paragraph{Equivalent to Serial Momentum...}
\begin{align*}
v_{t+1}&\leftarrow \beta v_T + (1-\beta)\nabla f(\theta_t) \\
\theta_{t+1}&\leftarrow \theta_t - \eta v_{t+1}\mbox{~(conceptual)}\\
\theta_{t+K}&\leftarrow \theta_t - \eta \sum_{i=1}^K v_{t+i}\mbox{~(real)}
\end{align*}
How to implement this?
\begin{align*}
v_{t+i} &= \beta^i v_t + (1-\beta) \sum_{j=0}^{i-1} \beta^{i-j} \nabla f(\theta_{t+j})\\
\sum_{i=1}^K v_{t+i}&= \frac{\beta(1-\beta^K)}{1-\beta} v_t + \sum_{i=0}^{K-1} (1-\beta^{K-i})\nabla f(\theta_{t+i})
\end{align*}
Can we directly maintain $p_{i, j} := \sum_{i=1}^j v_{t+i}$ and find a transition from $(\theta_i, p_{i-K, K})$ to $(\theta_{i+K}, p_{i, K})$ directly?? There could be some approximations, e.g., those based on the smoothness, or maybe we can do some interpolation. 


\paragraph{Anlysis of $\beta$ in scale problem}
\begin{align*}
    m_{t+1} = Q\left( Q\left(\beta m_t\right) + g_0 \right) \\
    \beta m_t \approx k \cdot s \\ 
    g_0 \ll s = \frac{\beta m_t}{k} \\
    m_t \approx \frac{1 - \beta^t}{1 - \beta} g_0
\end{align*}
which implies
\begin{align*}
    1 \ll \frac{\beta}{(1 - \beta)k}
\end{align*}
when $\beta$ decreases, this phenomenon is alleviated.

\subsection{Our algorithm: Hierarchical Summation}
\begin{align*}
g_{t, 0} & \leftarrow 0 \\
g_{t, i+1} & \leftarrow Q(g_{t, i} + \nabla \Tilde{f}(\theta_{t-1})) \\
m_{t} & \leftarrow Q(\beta m_{t-1} + g_{t, N}) \\
\theta_{t} & \leftarrow Q(\theta_{t-1} - \alpha m_t) \\
\end{align*}

\subsection{Convergence Theory}
\subsubsection{HSQ-SGD}
For SGD, our algorithm is simplified to this case
\begin{align*}
g_{t, 0} & \leftarrow 0 \\
g_{t, i+1} & \leftarrow Q(g_{t, i} + \nabla \Tilde{f}(\theta_{t-1})) \\
\theta_{t} & \leftarrow Q(\theta_{t-1} - \alpha g_{t, N}) 
\end{align*}

and we compare it with the basic quantized algorithm
\begin{align*}
\theta_{t} & \leftarrow Q(\theta_{t-1} - \alpha \nabla \Tilde{f}(\theta_{t-1})) 
\end{align*}

First, we focus on the \textbf{non-convex} case. we make following assumptions
\begin{enumerate}
    \item The objective function has unique global minimum $f(\theta^*)$.
    \item \textbf{Smoothness}: The objective $f(\theta)$ is continuous differentiable and L-smooth, i.e. $f(y) - f(x) \le \langle \nabla f(x), y - x \rangle + \frac{L}{2}\norm{x - y}^2$
    \item \textbf{Unbiasedness} for quantization function: $\Eb[Q(x)] = x$
    \item \textbf{Bounded variance (and second moments)}: $ \Eb[\norm{\nabla\Tilde{f}(\theta) - \nabla f(\theta)}^2] < \sigma^2 \quad \forall \theta$
\end{enumerate}

First, we need to clarify the property of $g_{t,i}$.
\begin{lemma}[first and second momentum of $g_{t,i}$]
    \label{lemma:g}
    \begin{align*}
        \Eb[g_{t, i}] & = i \nabla f(\theta_{t-1}) \\
        \Eb[\norm{g_{t, i}}^2] & \le \frac{i\delta_g^2d}{4} + i(i+2)\norm{\nabla f(\theta_{t-1})}^2 + i \sigma^2
    \end{align*}
\end{lemma}

Let $u_t = \theta_{t-1} - \alpha g_{t, N}$, consider $\theta_t$ and $u_t$, we have
\begin{align*}
    f(\theta_t) - f(u_t) \le \langle \nabla f(u_t), \theta_t - u_t \rangle + \frac{L}{2}\norm{\theta_t - u_t}^2
\end{align*}
Sine $\Eb[\theta_t] = u_t$, we have
\begin{align*}
    \Eb[f(\theta_t)] - f(u_t) \le \frac{L}{2}\norm{\theta_t - u_t}^2
\end{align*}
Using the most simple quantization error bound $\Eb[\norm{Q(x) - x}^2] \le \frac{\delta^2d}{4}$, we have
\begin{align*}
    \Eb[f(\theta_t)] - f(u_t) \le \frac{L}{2} \cdot \frac{\delta_p^2d}{4}
\end{align*}
Next, consider $u_t$ and $\theta_{t-1}$. In our algorithm, 
\begin{align*}
    f(u_t) - f(\theta_{t-1}) & \le \langle \nabla f(\theta_{t-1}), -\alpha g_{t, N} \rangle + \frac{\alpha^2L}{2} \norm{g_{t, N}}^2 \\
    \Eb[f(u_t)] - f(\theta_{t-1}) & \le -\alpha N \norm{\nabla f(\theta_{t-1})}^2 + \frac{\alpha^2L}{2} \norm{g_{t, N}}^2
\end{align*}
Substitute the bound of $\norm{g_{t, N}}$, we have
\begin{align}
    \label{eq:diff}
    \Eb[f(\theta_t)] - \Eb[f(\theta_{t-1})] \le -\alpha N (1 - \frac{(N+2)\alpha L}{2}) \norm{\nabla f(\theta_{t-1})}^2 + \frac{\alpha^2LN\sigma^2}{2} + \frac{1}{2}\alpha^2L\frac{N\delta_g^2d}{4} + \frac{1}{2}L\frac{\delta_p^2d}{4} 
\end{align}
Sum the result from 0 to T - 1, we have
\begin{align*}
    \alpha N (1 - \frac{(N + 2)\alpha L}{2}) \sum_{t=0}^{T-1} \Eb[\norm{\nabla f(\theta_t)}^2] \le f(\theta_0) - \Eb[f(\theta_T)] + T \cdot \left( \frac{\alpha^2LN\sigma^2}{2} + \frac{1}{2}\alpha^2L\frac{N\delta_g^2d}{4} + \frac{1}{2}L\frac{\delta_p^2d}{4}  \right)
\end{align*}
\begin{align*}
    \frac{1}{T} \sum_{t=0}^{T-1} \Eb[\norm{\nabla f(\theta_t)}^2]  \le  &
    \frac{2}{\alpha N(2 - (N+2)\alpha L)} \cdot \frac{f(\theta_0) - f^*}{T} \\
    & + \frac{1}{\alpha N(2 - (N+2)\alpha L)} \cdot \left( \alpha^2LN\sigma^2 + \alpha^2L\frac{N\delta_g^2d}{4} + L\frac{\delta_p^2d}{4} \right)
\end{align*}
While for basie quantized SGD, the convergence result is
\begin{align*}
    \frac{1}{T} \sum_{t=0}^{T-1} \Eb[\norm{\nabla f(\theta_t)}^2]  \le  &
    \frac{2}{\alpha (2 - \alpha L)} \cdot \frac{f(\theta_0) - f^*}{T} 
    + \frac{1}{\alpha (2 - \alpha L)} \cdot \left( \alpha^2L\sigma^2 
    +  L\frac{\delta_p^2d}{4} \right)
\end{align*}

When the two algorithm takes equal learning rate and $\delta_g \ll \delta_p$, the final stationary point of our algorithm is better. However, when $\alpha_\text{base} \approx N \alpha_\text{ours}$, the stationary point is similar.
Therefore, a large learning rate is important, and our algorithm plays a role in increasing the learning rate while not increasing the batch size synchronously.

Next, we focus the \textbf{strongly-convex} case. Based on the above assumptions, we make another assumption
\begin{enumerate}
    \item \textbf{Strong Convexity}: The objective $f(\theta)$ is $\mu$-strongly convex, i.e. $f(y) - f(x) \ge \langle \nabla f(x), y - x \rangle + \frac{\mu}{2}\norm{x - y}^2$
\end{enumerate}

By smoothness condition, we also have \ref{eq:diff}. And by strong convexity, we have
\begin{align}
    2\mu \left( f(\theta) - f_* \right) \le \norm{\nabla f(\theta)}^2,\,\forall \theta
\end{align}
Substitute into inequality \ref{eq:diff}, we finally have:
\begin{align}
    & \Eb[f(\theta_{t+1}) - f_*] - 
    \frac{\left( \alpha^2LN\sigma^2 + \alpha^2L\frac{N\delta_g^2d}{4} + L\frac{\delta_p^2d}{4} \right)}{2\mu\alpha N(2 - (N+2)\alpha L)} \\
    \le & \left( 1 - N\alpha\mu\left( 2 - (N+2)\alpha L\right)\right)
    \left( \Eb[f(\theta_{t}) - f_*] - 
    \frac{\left( \alpha^2LN\sigma^2 + \alpha^2L\frac{N\delta_g^2d}{4} + L\frac{\delta_p^2d}{4} \right)}{2\mu\alpha N(2 - (N+2)\alpha L)} \right)
\end{align}
While for basie quantized SGD, the strong convex convergence result is
\begin{align*}
    & \Eb[f(\theta_{t+1}) - f_*] - 
    \frac{\left( \alpha^2L\sigma^2 
    +  L\frac{\delta_p^2d}{4} \right)}{2\mu\alpha (2 - \alpha L)} \\
    \le & \left( 1 - \alpha\mu( 2 - \alpha L)\right)
    \left( \Eb[f(\theta_{t}) - f_*] - 
    \frac{\left( \alpha^2L\sigma^2 
    +  L\frac{\delta_p^2d}{4} \right)}{2\mu\alpha (2 - \alpha L)} \right)
\end{align*}

\subsubsection{Basic Quantized SGDM}
For SGDM, consider the following algorithm
\begin{align*}
m_{t} & \leftarrow Q(\beta m_{t-1} + \nabla \Tilde{f}(\theta_{t-1})) \\
\theta_{t} & \leftarrow Q(\theta_{t-1} - \alpha m_t) \\
\end{align*}
We call this algorithm the basic quantized SGDM. The convergence of this algorithm has still not been given. 

\paragraph{Preparations}
For convenience, we define some notations 
\begin{align}
    u_{t} = \beta m_{t-1} + \nabla \Tilde{f}(\theta_{t-1}) \\
    v_{t} = \sum_{i=1}^T \beta^{t-i} \nabla \Tilde{f}(\theta_{i-1})
\end{align}
Directly, we have $\Eb_{Q_t}[m_t] = u_t,\,\Eb[m_t] = \Eb[u_t] = \Eb[v_t]$. 
Next, we define an auxiliary sequences ${z_t}$ which is critical for the proof.
\begin{align}
    z_t = \begin{cases}
    \theta_0,\, & t = 0 \\ 
    \frac{1}{1 - \beta}\theta_t - \frac{\beta}{1 - \beta}\theta_{t-1},\, & \text{otherwise}
    \end{cases}
\end{align}
Subsequently, we compute the moments of $z_{t+1} - z_t$ and get
\begin{align}
    z_{t+1} - z_{t} & = \frac{1}{1 - \beta} (\theta_{t+1} - \theta_t) - \frac{\beta}{1 - \beta}(\theta_t - \theta_{t-1}) \\
    \Eb[z_{t+1} - z_{t}] & = \frac{-\alpha}{1 - \beta} \nabla f(\theta_t) \\
    \Eb[\norm{z_{t+1} - z_{t}}^2] 
    & \le  \left(\frac{\alpha}{1-\beta}\right)^2 \left( \Eb[\norm{\nabla f(\theta_t)}^2] + \sigma^2 + \frac{\delta_m^2d}{4} \right) + \frac{1 + \beta^2}{(1 - \beta)^2} \frac{\delta_p^2d}{4}
\end{align}
Note that the quantity $\Eb[\norm{z_{t+1} - z_{t}}^2]$ are composed by three parts: the variance of stochastic gradient, quantized momentums and quantized parameters which are independent from each other.


\paragraph{Convex Case}
For \textbf{convex} case, suppose that $\theta_*$ is the optimal parameter and $f_* = f(\theta_*)$ is the minimal objective value. First, we have
\begin{align}
    \norm{z_{t+1} - \theta_*}^2 & = \norm{z_{t} - \theta_*}^2 
    + 2 \left\langle z_t - \theta_*, z_{t+1} - z_t \right\rangle + \norm{z_{t+1} - z_t}^2
\end{align}
Take expectation over the randomness in the \text{(t+1)}-th step, we have
\begin{align}
    \Eb[\norm{z_{t+1} - \theta_*}^2] & = \norm{z_{t} - \theta_*}^2 
    - \frac{2\alpha}{1-\beta} \left\langle z_t - \theta_*, \nabla f(\theta_t) \right\rangle + \Eb[\norm{z_{t+1} - z_t}^2] \\
    & = \norm{z_{t} - \theta_*}^2 
    - \frac{2\alpha}{1-\beta} \left\langle \theta_t - \theta_*, \nabla f(\theta_t) \right\rangle \\
    & - \frac{2\alpha\beta}{(1-\beta)^2} \left\langle \theta_t - \theta_{t-1}, \nabla f(\theta_t)
    \right\rangle + \Eb[\norm{z_{t+1} - z_t}^2]
\end{align}
Since $f$ is continuously differentiable and L-smooth, we have some inequalities. Substitute them and get
\begin{align}
    \Eb[\norm{z_{t+1} - \theta_*}^2] 
    & \le \norm{z_{t} - \theta_*}^2 
    - \frac{2\alpha(1 - \rho)}{L(1-\beta)} \norm{\nabla f(\theta_t)}^2 
    - \frac{2\alpha\rho}{1-\beta} (f(\theta_t) - f_*)\\
    & \frac{\alpha\rho}{L(1-\beta)} \norm{\nabla f(\theta_t)}^2  - \frac{2\alpha\beta}{(1-\beta)^2} (f(\theta_t) - f(\theta_{t-1}))
    + \Eb[\norm{z_{t+1} - z_t}^2]
\end{align}
Substitute the bound of $\Eb[\norm{z_{t+1} - z_t}^2]$ and collect the terms, we get
\begin{align}
    & \left( \frac{2\alpha\rho}{1-\beta} + \frac{2\alpha\beta}{(1-\beta)^2} \right) (f(\theta_t) - f_*) + \Eb[\norm{z_{t+1} - \theta_*}^2] \\
    \le &  \frac{2\alpha\beta}{(1-\beta)^2} \left( f(\theta_{t-1}) - f_*\right) 
    + \norm{z_t - \theta_*}^2 
    + \left( \frac{\alpha^2}{(1 - \beta)^2}  - \frac{\alpha(2 - \rho)}{L(1-\beta)} \right) \norm{\nabla f(\theta_t)}^2  \\
    & + \left(\frac{\alpha}{1-\beta}\right)^2 \left(\sigma^2 + \frac{\delta_m^2d}{4} \right) + \frac{1 + \beta^2}{(1 - \beta)^2} \frac{\delta_p^2d}{4}
\end{align}
when $\alpha$ satisfies the condition $ \frac{\alpha^2}{(1 - \beta)^2}  - \frac{\alpha(2 - \rho)}{L(1-\beta)} \le 0$, i.e. $ 0 \le \alpha \le \frac{(1 - \beta)(2 - \rho)}{L}$, the term about $\norm{\nabla f(\theta_t)}^2$ is non-positive, thus we have
\begin{align}
    & \left( \frac{2\alpha\rho}{1-\beta} + \frac{2\alpha\beta}{(1-\beta)^2} \right) (f(\theta_t) - f_*) + \Eb[\norm{z_{t+1} - \theta_*}^2] \\
    \le &  \frac{2\alpha\beta}{(1-\beta)^2} \left( f(\theta_{t-1}) - f_*\right) 
    + \norm{z_t - \theta_*}^2 
    + \left(\frac{\alpha}{1-\beta}\right)^2 \left(\sigma^2 + \frac{\delta_m^2d}{4} \right) + \frac{1 + \beta^2}{(1 - \beta)^2} \frac{\delta_p^2d}{4}
\end{align}
Denote $M = \left(\frac{\alpha}{1-\beta}\right)^2 \left(\sigma^2 + \frac{\delta_m^2d}{4} \right) + \frac{1 + \beta^2}{(1 - \beta)^2} \frac{\delta_p^2d}{4}$.
Summing this inequality from 0 to $T - 1$ and taking full expectation gives
\begin{align}
    & \frac{2\alpha\rho}{1-\beta} \sum_{i=0}^{T-1} \Eb[f(\theta_i) - f_*] 
    + \sum_{i=0}^{T-1} \left( \frac{2\alpha\beta}{(1-\beta)^2} \Eb[f(\theta_{i}) - f_*] + \Eb[\norm{z_{i+1} - \theta_*}^2]\right) \\
    \le & \sum_{i=0}^{T-1}  \left( \frac{2\alpha\beta}{(1-\beta)^2} \Eb[f(\theta_{i-1}) - f_*] + \Eb[\norm{z_{i} - \theta_*}^2]\right) + T\cdot M
\end{align}
which implies that
\begin{align}
    \frac{2\alpha\rho}{1-\beta} \sum_{i=0}^{T-1} \Eb[f(\theta_i) - f_*] 
    & \le \frac{2\alpha\beta}{(1-\beta)^2} (f(\theta_0) - f_*) + \norm{\theta_0 - \theta_*}^2 + T\cdot M
\end{align}
note that we define $\theta_{-1} = \theta_0$ for technical reasons. Since $f$ is \textbf{convex}, we have $T f(\Bar{{\theta}}_T) \le \frac{1}{T}\sum_{i=0}^{T-1} f(\theta_i))$.
Subsequently we have
\begin{align}
    \Eb[f(\Bar{{\theta}}_T) - f_*] & \le \frac{1}{T}\left( \frac{\beta}{\rho(1-\beta)}(f(\theta_0) - f_*) + \frac{1-\beta}{2\alpha\rho}\norm{\theta_0 - \theta_*}^2 \right) \\
    & + \frac{1-\beta}{2\alpha\rho}M
\end{align}
Substituting $M$ gives
\begin{align}
    \Eb[f(\Bar{{\theta}}_T) - f_*] & \le \frac{1}{T}\left( \frac{\beta}{\rho(1-\beta)}(f(\theta_0) - f_*) + \frac{1-\beta}{2\alpha\rho}\norm{\theta_0 - \theta_*}^2 \right) \\
    & + \frac{\alpha \sigma^2}{2\rho(1-\beta)} + \frac{\alpha\delta_m^2d}{8\rho(1-\beta)}
    + \frac{(1+\beta^2\delta_p^2d)}{8\alpha\rho(1-\beta)}
\end{align}
Finally, when $\alpha \in (0, \frac{1-\beta}{L}]$, we can take $\rho=1$ and use L-smooth condition again, which gives
\begin{align}
    \Eb[f(\Bar{{\theta}}_T) - f_*] & \le \frac{1}{2T}\left( \frac{L\beta}{1-\beta} + \frac{1-\beta}{\alpha} \right) \norm{\theta_0 - \theta_*}^2\\
    & + \frac{\alpha \sigma^2}{2(1-\beta)} + \frac{\alpha\delta_m^2d}{8(1-\beta)}
    + \frac{(1+\beta^2)\delta_p^2d}{8\alpha(1-\beta)}
\end{align}

\paragraph{Non-convex Case}
TODO

\subsubsection{HSQ-SGDM}
\begin{align*}
g_{t, 0} & \leftarrow 0 \\
g_{t, i+1} & \leftarrow Q(g_{t, i} + \nabla \Tilde{f}(\theta_{t-1})) \\
m_{t} & \leftarrow Q(\beta m_{t-1} + g_{t, N}) \\
\theta_{t} & \leftarrow Q(\theta_{t-1} - \alpha m_t) \\
\end{align*}
                 
\paragraph{Preparations}
For convenience, we define similar notations 
\begin{align}
    u_{t} = \beta m_{t-1} + g_{t,N} \\
    v_{t} = \sum_{i=1}^T \beta^{t-i} g_{t,N}
\end{align}
Directly, we have $\Eb_{Q_t}[m_t] = u_t,\,\Eb[m_t] = \Eb[u_t] = \Eb[v_t]$. 
Next, we consider the moments of auxiliary sequences ${z_t}$ and have
\begin{align}
    z_{t+1} - z_{t} & = \frac{1}{1 - \beta} (\theta_{t+1} - \theta_t) - \frac{\beta}{1 - \beta}(\theta_t - \theta_{t-1}) \\
    \Eb[z_{t+1} - z_{t}] & = \frac{-\alpha N}{1 - \beta} \nabla f(\theta_t) \\
    \Eb[\norm{z_{t+1} - z_{t}}^2] 
    & \le  \left(\frac{\alpha}{1-\beta}\right)^2 \left( \Eb[\norm{g_{t,N}}^2] + \sigma^2 + \frac{\delta_m^2d}{4} \right) + \frac{1 + \beta^2}{(1 - \beta)^2} \frac{\delta_p^2d}{4}
\end{align}
and the analysis in HSQ-SGD tells us
\begin{align}
    \label{eq:bound-of-gtN}
    \Eb[\norm{g_{t,N}}^2] & \le \frac{N\delta_g^2d}{4} + N(N+2)\norm{\nabla f(\theta_{t-1})}^2 + N\sigma^2
\end{align}
Substituting \ref{eq:bound-of-gtN} gives 
\begin{align}
    \label{eq:hsq-bound-of-z-diff}
    \Eb[\norm{z_{t+1} - z_{t}}^2] 
    & \le  \left(\frac{\alpha}{1-\beta}\right)^2 \left( N(N+2)\Eb[\norm{\nabla f(\theta_t)}^2] + N\sigma^2 \right) \\
    & + \left(\frac{\alpha}{1-\beta}\right)^2 \left( \frac{N\delta_g^2d}{4} 
    + \frac{\delta_m^2d}{4} \right) + \frac{1 + \beta^2}{(1 - \beta)^2} \frac{\delta_p^2d}{4}
\end{align}

\paragraph{Convex Case}
For \textbf{convex} case, suppose that $\theta_*$ is the optimal parameter and $f_* = f(\theta_*)$ is the minimal objective value. First, we have
\begin{align}
    \norm{z_{t+1} - \theta_*}^2 & = \norm{z_{t} - \theta_*}^2 
    + 2 \left\langle z_t - \theta_*, z_{t+1} - z_t \right\rangle + \norm{z_{t+1} - z_t}^2
\end{align}
Take expectation over the randomness in the \text{(t+1)}-th step, we have
\begin{align}
    \Eb[\norm{z_{t+1} - \theta_*}^2] & = \norm{z_{t} - \theta_*}^2 
    - \frac{2\alpha N}{1-\beta} \left\langle z_t - \theta_*, \nabla f(\theta_t) \right\rangle + \Eb[\norm{z_{t+1} - z_t}^2] \\
    & = \norm{z_{t} - \theta_*}^2 
    - \frac{2\alpha N}{1-\beta} \left\langle \theta_t - \theta_*, \nabla f(\theta_t) \right\rangle \\
    & - \frac{2\alpha\beta N}{(1-\beta)^2} \left\langle \theta_t - \theta_{t-1}, \nabla f(\theta_t)
    \right\rangle + \Eb[\norm{z_{t+1} - z_t}^2]
\end{align}
Since $f$ is continuously differentiable and L-smooth, we have some inequalities. Substitute them and get
\begin{align}
    \Eb[\norm{z_{t+1} - \theta_*}^2] 
    & \le \norm{z_{t} - \theta_*}^2 
    - \frac{2\alpha N(1 - \rho)}{L(1-\beta)} \norm{\nabla f(\theta_t)}^2 
    - \frac{2\alpha N\rho}{1-\beta} (f(\theta_t) - f_*)\\
    & \frac{\alpha N\rho}{L(1-\beta)} \norm{\nabla f(\theta_t)}^2  - \frac{2\alpha N\beta}{(1-\beta)^2} (f(\theta_t) - f(\theta_{t-1}))
    + \Eb[\norm{z_{t+1} - z_t}^2]
\end{align}
For the last term, denote $M = \left(\frac{\alpha}{1-\beta}\right)^2 \left( N\sigma^2 + \frac{N\delta_g^2d}{4} + \frac{\delta_m^2d}{4} \right) + \frac{1 + \beta^2}{(1 - \beta)^2} \frac{\delta_p^2d}{4}$. Substitute \ref{eq:hsq-bound-of-z-diff} into last inequality and collect the terms, we get
\begin{align}
    & \left( \frac{2\alpha N\rho}{1-\beta} + \frac{2\alpha N\beta}{(1-\beta)^2} \right) (f(\theta_t) - f_*) + \Eb[\norm{z_{t+1} - \theta_*}^2] \\
    \le &  \frac{2\alpha N\beta}{(1-\beta)^2} \left( f(\theta_{t-1}) - f_*\right) 
    + \norm{z_t - \theta_*}^2 
    + \left( \frac{\alpha^2N(N+2)}{(1 - \beta)^2}  - \frac{\alpha N(2 - \rho)}{L(1-\beta)} \right) \norm{\nabla f(\theta_t)}^2 + M
\end{align}
when $\alpha$ satisfies the condition $ \frac{\alpha^2N(N+2)}{(1 - \beta)^2}  - \frac{\alpha N(2 - \rho)}{L(1-\beta)} \le 0$, i.e. $ 0 \le \alpha \le \frac{(1 - \beta)(2 - \rho)}{(N+2)L}$, the term about $\norm{\nabla f(\theta_t)}^2$ is non-positive, thus we have
\begin{align}
    & \left( \frac{2\alpha N\rho}{1-\beta} + \frac{2\alpha N\beta}{(1-\beta)^2} \right) (f(\theta_t) - f_*) + \Eb[\norm{z_{t+1} - \theta_*}^2] \\
    \le &  \frac{2\alpha N\beta}{(1-\beta)^2} \left( f(\theta_{t-1}) - f_*\right) 
    + \norm{z_t - \theta_*}^2 + M
\end{align}
Summing this inequality from 0 to $T - 1$ and taking full expectation gives
\begin{align}
    & \frac{2\alpha N\rho}{1-\beta} \sum_{i=0}^{T-1} \Eb[f(\theta_i) - f_*] 
    + \sum_{i=0}^{T-1} \left( \frac{2\alpha N\beta}{(1-\beta)^2} \Eb[f(\theta_{i}) - f_*] + \Eb[\norm{z_{i+1} - \theta_*}^2]\right) \\
    \le & \sum_{i=0}^{T-1}  \left( \frac{2\alpha N\beta}{(1-\beta)^2} \Eb[f(\theta_{i-1}) - f_*] + \Eb[\norm{z_{i} - \theta_*}^2]\right) + T\cdot M
\end{align}
which implies that
\begin{align}
    \frac{2\alpha N\rho}{1-\beta} \sum_{i=0}^{T-1} \Eb[f(\theta_i) - f_*] 
    & \le \frac{2\alpha N\beta}{(1-\beta)^2} (f(\theta_0) - f_*) + \norm{\theta_0 - \theta_*}^2 + T\cdot M
\end{align}
Since $f$ is \textbf{convex}, we have $T f(\Bar{{\theta}}_T) \le \frac{1}{T}\sum_{i=0}^{T-1} f(\theta_i))$.
Subsequently we have
\begin{align}
    \Eb[f(\Bar{{\theta}}_T) - f_*] & \le \frac{1}{T}\left( \frac{\beta}{\rho(1-\beta)}(f(\theta_0) - f_*) + \frac{1-\beta}{2\alpha N\rho}\norm{\theta_0 - \theta_*}^2 \right) \\
    & + \frac{1-\beta}{2\alpha N\rho}M
\end{align}
Finally, when $\alpha \in (0, \frac{1-\beta}{(N+2)L}]$, we can take $\rho=1$, use L-smooth condition again and substitute $M$, which gives
\begin{align}
    \Eb[f(\Bar{{\theta}}_T) - f_*] & \le \frac{1}{2T}\left( \frac{L\beta}{1-\beta} + \frac{1-\beta}{\alpha N} \right) \norm{\theta_0 - \theta_*}^2\\
    & + \frac{\alpha \sigma^2}{2(1-\beta)} 
    + \frac{\alpha\delta_g^2d}{8(1-\beta)}
    + \frac{\alpha\delta_m^2d}{8N(1-\beta)}
    + \frac{(1+\beta^2)\delta_p^2d}{8\alpha N(1-\beta)}
\end{align}
While for basie quantized SGDM, the convex convergence result is
\begin{align*}
    \Eb[f(\Bar{{\theta}}_T) - f_*] & \le \frac{1}{2T}\left( \frac{L\beta}{1-\beta} + \frac{1-\beta}{\alpha} \right) \norm{\theta_0 - \theta_*}^2\\
    & + \frac{\alpha \sigma^2}{2(1-\beta)} + \frac{\alpha\delta_m^2d}{8(1-\beta)}
    + \frac{(1+\beta^2)\delta_p^2d}{8\alpha(1-\beta)}
\end{align*}

\paragraph{Non-convex Case} TODO


